Learning Setup Policies: Reliable Transition Between Locomotion Behaviours

Dynamic platforms that operate over many unique terrain conditions typically require many behaviours. To transition safely, there must be an overlap of states between adjacent controllers. We develop a novel method for training setup policies that bridge the trajectories between pre-trained Deep Reinforcement Learning (DRL) policies. We demonstrate our method with a simulated biped traversing a difficult jump terrain, where a single policy fails to learn the task, and switching between pre-trained policies without setup policies also fails. We perform an ablation of key components of our system, and show that our method outperforms others that learn transition policies. We demonstrate our method with several difficult and diverse terrain types, and show that we can use setup policies as part of a modular control suite to successfully traverse a sequence of complex terrains. We show that using setup policies improves the success rate for traversing a single difficult jump terrain (from 51.3% success rate with the best comparative method to 82.2%), and traversing a random sequence of difficult obstacles (from 1.9% without setup policies to 71.2%).

==> diff.tex <==
%DIF 1d1
%DIF LATEXDIFF DIFFERENCE FILE
%DIF DEL old_main.tex   Wed Jul 27 09:00:42 2022
%DIF ADD main.tex       Wed Jul 27 08:54:27 2022
%DIF < 
%DIF -------
\title{\LARGE \bf
%Setup Policies For Composing Locomotion Behaviours
% Learning Setup Policies for Transitioning Between Locomotion Policies
Learning Setup Policies: Reliable Transition
\\ Between Locomotion Behaviours
% Learning a Reliable Setup Policy for Transitioning Between Locomotion Behaviours
% Learning to Reliably Transition Between Locomotion Policies
}
% \title{\LARGE \bf
% Setup Before Switching: Learning Transition Policies for Combining DRL Policies 
% }

\author{Brendan Tidd$^{1,2}$, Nicolas Hudson\DIFdelbegin \DIFdel{$^{2}$}\DIFdelend \DIFaddbegin \DIFadd{$^{3}$}\DIFaddend , Akansel Cosgun\DIFdelbegin \DIFdel{$^{3}$ }\DIFdelend \DIFaddbegin \DIFadd{$^{4}$ }\DIFaddend and J\"{u}rgen Leitner\DIFdelbegin \DIFdel{$^{4}$}\DIFdelend \DIFaddbegin \DIFadd{$^{5,6}$}\DIFaddend % <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Queensland University of Technology (QUT), Australia}%
\thanks{$^{2}$Robotics and Autonomous Systems Group, CSIRO, Pullenvale, QLD 4069, Australia \newline Email: brendan.tidd@data61.csiro.au}
\DIFdelbegin %DIFDELCMD < \thanks{$^{3}$Monash University, Australia}%%%
\DIFdelend \DIFaddbegin \thanks{$^{3}$Amazon, United States}\DIFaddend %
\DIFdelbegin %DIFDELCMD < \thanks{$^{4}$LYRO Robotics Pty Ltd, Australia}%%%
\DIFdelend \DIFaddbegin \thanks{$^{4}$Deakin University, Australia}%DIF > 
\thanks{$^{5}$Monash University, Australia}%DIF > 
\thanks{$^{6}$LYRO Robotics Pty Ltd, Australia}\DIFaddend %
%\thanks{$^{4}$Australian Centre for Robotic Vision}%
}
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
\providecommand{\DIFmodbegin}{} %DIF PREAMBLE
\providecommand{\DIFmodend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF LISTINGS PREAMBLE %DIF PREAMBLE
\RequirePackage{listings} %DIF PREAMBLE
\RequirePackage{color} %DIF PREAMBLE
\lstdefinelanguage{DIFcode}{ %DIF PREAMBLE
%DIF DIFCODE_UNDERLINE %DIF PREAMBLE
  moredelim=[il][\color{red}\sout]{\%DIF\ <\ }, %DIF PREAMBLE
  moredelim=[il][\color{blue}\uwave]{\%DIF\ >\ } %DIF PREAMBLE
} %DIF PREAMBLE
\lstdefinestyle{DIFverbatimstyle}{ %DIF PREAMBLE
	language=DIFcode, %DIF PREAMBLE
	basicstyle=\ttfamily, %DIF PREAMBLE
	columns=fullflexible, %DIF PREAMBLE
	keepspaces=true %DIF PREAMBLE
} %DIF PREAMBLE
\lstnewenvironment{DIFverbatim}{\lstset{style=DIFverbatimstyle}}{} %DIF PREAMBLE
\lstnewenvironment{DIFverbatim*}{\lstset{style=DIFverbatimstyle,showspaces=true}}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

\begin{document}

\maketitle
\thispagestyle{empty}
\pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
\label{sec:abstract}
Dynamic platforms that operate over many unique terrain conditions typically require many behaviours. To transition safely, there must be an overlap of states between adjacent controllers. We develop a novel method for training setup policies that bridge the trajectories between pre-trained Deep Reinforcement Learning (DRL) policies. We demonstrate our method with a simulated biped traversing a difficult jump terrain, where a single policy fails to learn the task, and switching between pre-trained policies without setup policies also fails. We perform an ablation of key components of our system, and show that our method outperforms others that learn transition policies. We demonstrate our method with several difficult and diverse terrain types, and show that we can use setup policies as part of a modular control suite to successfully traverse a sequence of complex terrains. We show that using setup policies improves the success rate for traversing a single difficult jump terrain (from \DIFdelbegin \DIFdel{1.5}\DIFdelend \DIFaddbegin \DIFadd{51.3}\DIFaddend $\%$ success rate \DIFdelbegin \DIFdel{without setup policies to 82}\DIFdelend \DIFaddbegin \DIFadd{with the best comparative method to 82.2}\DIFaddend $\%$), and traversing a random sequence of difficult obstacles (from 1.9$\%$ without setup policies to 71.2$\%$).


% \textbf{why do I care?}
% , as it may not be possible to safely switch between controllers outside of the overlapping states.
\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:introduction}

Bipedal robots have the capability to cover a span of terrains that humans can traverse. This makes bipeds an appealing locomotion option for robots in human environments. It is impractical, however, to design a single controller that works over all required environments, particularly if all conditions are not known a priori. For robots to be able to perform a number of diverse behaviours, it is desirable for a control suite to be modular, where any number of behaviours can be added with minimal retraining.

% included in the control repertoire. 
% Ideally, as new conditions are identified and new controllers become available, the new behaviours can be added to the control suite with minimal retraining.

Deep Reinforcement Learning (DRL) is an appealing method for developing visuo-motor behaviours for legged platforms. However, such DRL policies are usually trained on the terrain they are expected to operate, though it is unlikely that the agent would have access to a complete set of terrain conditions during policy training before deployment. Controllers for dynamic platforms are typically developed and tuned with safety harnesses and human supervisors in order to minimise potential damage to the robot and the environment. These restrictions limit the development of controllers over an exhaustive collection of terrain conditions. Furthermore, modifying controllers that have already been tuned is costly, for example DRL methods \DIFaddbegin \DIFadd{that are trained for discrete terrain types }\DIFaddend typically require retraining if new \DIFdelbegin \DIFdel{terrains are introduced }\DIFdelend \DIFaddbegin \DIFadd{terrain variations are introduced \mbox{%DIFAUXCMD
\cite{peng_dynamic_2015}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend . We propose training a \textit{setup policy} to transition between two pre-trained policies targeting different terrains.

A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over if controllers are switched when the robot is not in a safe region for the subsequent controller. Figure~\ref{fig:fig1} shows our primary contribution: a setup policy that prepares the robot for the necessary controller to traverse the upcoming terrain obstacle. With our method, we can transition between existing behaviours, allowing pre-trained DRL policies to be combined. 

% We propose a modular approach to developing a control suite for a biped expected to traverse a number of difficult terrain artifacts, where all terrain conditions are not known when training each module. A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over. Figure~\ref{fig:fig1} shows our primary contribution: a setup policy that prepares the robot for the upcoming terrain artifact. With our method, we can safely transition between behaviours that are developed separately, such that any number of pre-trained DRL policies can be combined, without any re-training of low level policies.  

\begin{figure}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth,natwidth=610,natheight=642]{images/Fig1.png}
\includegraphics[width=\columnwidth]{images/Fig1.png}
% \includegraphics[width=\columnwidth]{images/Fig1_err.png}
\hfill
\caption{As the robot approaches a difficult terrain artifact, it must move into position for target policy $i$. The trajectory of the walking policy $j$ (shown with a blue line), does not intersect with the trajectory of the target policy $i$ (green line). Our setup policy provides a trajectory that prepares the robot for the upcoming target policy (orange line).}
\label{fig:fig1}
% \vspace{-3mm}
\end{figure}
% How can we leverage subpolicy learning to improve learning outcomes?
Our contributions are as follows:
\begin{itemize}
    \item Using pre-trained policies, we develop \textbf{setup policies} that significantly improve the success rate from transitioning from a default walking policy to a target policy\DIFdelbegin \DIFdel{(from 1.5$\%$ success rate without setup policies to 82$\%$ for a difficult 0.5m jump)}\DIFdelend . The setup policy also learns when to switch to the target policy. 
    \item We introduce a novel reward, called \textbf{Advantage Weighted Target Value}, guiding the robot towards the target policy.
    \item We show that we can use setup policies with several difficult terrain types, allowing for a modular control suite, combining behaviours that have been trained separately without any retraining of low level policies.
\end{itemize}

% The organization of this paper is as follows. After reviewing the relevant literature in Sec~\ref{sec:related_work}, we define the problem in Sec~\ref{sec:problem}, the learning algorithm in Sec~\ref{sec:ppo}, and our method for developing setup policies in Sec~\ref{sec:setup}. Our experimental results and comparisons are shown in Sec~\ref{sec:experiments}. Finally, we conclude with a brief discussion in Sec~\ref{sec:conclusion}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:related_work}
% Related work should also be story, starting from the start of the problem, highlighting what is missing, and refining to the specific paper that is closest to ours. Goal is to find gaps, start broad, and funnel into specifics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Deep reinforcement learning (DRL) has demonstrated impressive results for locomotion tasks in recent works~\cite{heess_emergence_2017, peng_deeploco_2017, peng_deepmimic_2018, xie_allsteps_2020}. Typically DRL policies optimise a single reward function, as new environments and behaviours are introduced costly retraining is required. Single policies have demonstrated locomotion over various terrains for simple 2D cases \cite{song_recurrent_2018}, and impressive quadruped behaviours \cite{lee_learning_2020, rudin_learning_2021}, however, for many scenarios multiple policies are often required. Furthermore, developing a single policy to perform multiple behaviours can degrade the performance of each behaviour~\cite{lee_robust_2019}.

Hierarchical reinforcement learning (HRL) offers flexibility through architecture, by training all segments of the hierarchy concurrently~\cite{sutton_between_1999, bacon_option-critic_2018, frans_meta_2018,peng_deeploco_2017}, or training parts of the hierarchy separately~\cite{merel_hierarchical_2019},~\cite{lee_composing_2019}.  When trained together, HRL can improve task level outcomes, such as steering and object tracking~\cite{peng_deeploco_2017}, or improve learning efficiency by reusing low level skills across multiple high level tasks~\cite{frans_meta_2018}. When trained separately, low level controllers can be refined efficiently using prior knowledge, such as by utilising motion capture data~\cite{peng_deepmimic_2018, merel_hierarchical_2019, peng_mcp_2019} or behavioural cloning~\cite{strudel_learning_2020}. For robotics applications it may be difficult to develop controllers for multiple behaviours simultaneously. Using pre-trained primitives can break up a large difficult problem into smaller solvable sub-problems~\cite{schaal_dynamic_2006}.

Using pre-trained policies requires suitable handling of transitions between behaviours. Faloutsos et al.~\cite{faloutsos_composable_2001} \DIFdelbegin \DIFdel{learns }\DIFdelend \DIFaddbegin \DIFadd{learn }\DIFaddend pre and post-conditions for each controller, such that switching only occurs when these conditions have been satisfied. DeepMimic by Peng et al.~\cite{peng_deepmimic_2018} combines pre-trained behaviours learned from motion capture, with reliance on a phase variable to determine when one behaviour has been completed. Policy sketches introduce a hierarchical method that uses task specific policies, with each task performed in sequence~\cite{andreas_modular_2017}. CompILE uses soft boundaries between task segments~\cite{kipf_compile_2019}. Work by Peng et al.~\cite{peng_terrain-adaptive_2016} trains several actor-critic control policies, modulated by the highest critic value in a given state. For these examples there must be a reasonable state overlap between controllers.

Other methods that combine pre-trained behaviours learn latent representations of skills~\cite{pertsch_accelerating_2020} or primitives~\cite{ha_distilling_2020}, enabling interpolation in the latent space. From an offline dataset of experience, Pertsch et al.~\cite{pertsch_accelerating_2020} were able to combine low level controllers in manipulation tasks and locomotion for a multi-legged agent. \DIFaddbegin \DIFadd{In our previous work~\mbox{%DIFAUXCMD
\cite{tidd_learning_2021}}\hspace{0pt}%DIFAUXCMD
, we learn when to switch between low level primitives for a simulated biped using data collected by randomly switching between behaviours. }\DIFaddend Ha et al.~\cite{ha_distilling_2020} utilise motion capture to learn latent representations of primitives, then use model predictive control to navigate with a high dimensional humanoid. The FeUdal approach learns a master policy that modulates
low-level policies using a learned goal signal~\cite{vezhnevets_feudal_2017}. \DIFdelbegin \DIFdel{Work }\DIFdelend \DIFaddbegin \DIFadd{Interpolation between behaviours yields natural transitions~\mbox{%DIFAUXCMD
\cite{xu_hierarchical_2020}}\hspace{0pt}%DIFAUXCMD
. The work }\DIFaddend by Peng et al.~\cite{peng_mcp_2019} combines pre-trained policies using a gating function that learns a multiplicative combination of \DIFdelbegin \DIFdel{actions. In our previous work~\mbox{%DIFAUXCMD
\cite{tidd_learning_2021}}\hspace{0pt}%DIFAUXCMD
, we learn when to switch between low level primitives for a simulated biped using data collected by randomly switching between behaviours . Interpolation between behaviours yields natural transitions~\mbox{%DIFAUXCMD
\cite{xu_hierarchical_2020}}\hspace{0pt}%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{behaviours to generate smooth actions}\DIFaddend . Yang et al.~\cite{yang_multi_2020} learn a gating neural network to blend several separate expert neural network policies to perform trotting, steering, and fall recovery in real-world experiments with a quadruped. Da et al.~\cite{da_supervised_2017} use supervised learning to train a control policy for a biped from several manually derived controllers to perform periodic and transitional gaits on flat and sloped ground. In each of these approaches, experience from all behaviours must be available during training. 

For dynamic platforms, where separate controllers occupy different subsets of the state, changing behaviours may result in instability if there is no overlap between controllers. Lee et al.~\cite{lee_composing_2019} learn a proximity predictor to train a transition policy to guide an agent to the initial state required by the next controller. Locomotion experiments are demonstrated with a 2D planar walker, where learning occurs by training with all terrain conditions. We show that our method performs more reliably (with a higher success rate), despite training with experience from a single terrain type. Our setup policies learn to transition between complex behaviours with a 3D biped in a simulation environment using a depth image to perceive the terrain. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Berkencamp, and mace use values to estimate when to use controllers.
% Composing paper. Something more specific about our method: advantage weighted value, this is a primary contribution. Training on sample only. Scaling to any number of policies, only needing data to train classifier, (no training of policies on anything but samples).


% sequential decision making tasks
% with greater sample efficiency than their non-hierarchical counterparts because hierarchical agents can break down tasks into sets of subtasks that only require short
% sequences of decisions.LEARNING MULTI-LEVEL HIERARCHIES WITH
% HINDSIGHT Andrew Levy , Hierarchical Actor-Critic (HAC), . Yet, learning multiple
% levels of policies in parallel is hard because it is inherently unstable: changes in
% a policy at one level of the hierarchy may cause changes in the transition and reward functions at higher levels in the hierarchy, making it difficult to jointly learn
% multiple levels of policies.  The main idea behind HAC is to train each level of the
% hierarchy independently of the lower levels by training each level as if the lower
% level policies are already optimal.

% HIRO Data-Efficient Hierarchical Reinforcement Learning Ofir Nachum - Use reward relabeling - High level give goals to low level. rewards from the environment are reused, temporal abstraction, off-policy.


% The first category lets a high-level policy select a low-level skill to execute [13, 14, 15, 28],
% which we refer to as the selector methods. In the second category, a subgoal is set for the low level by
% high-level policies [8, 9, 11, 10, 25], which we refer to as subgoal-based methods.

% % \subsection{Hierarchical RL}

% % \subsection{Transition Policies and Modular RL}
% % \textbf{ TODO Transition papers
% \begin{itemize}
%     \item sutton \cite{Sutton2017ReinforcementA.G.}
%     \item HRL \cite{sutton_between_1999} - introduces options, a framework for splitting mdp into temporally abstracted options.
%     \item m, HRL with Advantage function-based Auxiliary Rewards \cite{li et al} - Use the advantage of the high level policy as dense reward signal for an otherwise sparse reward problem,  improving pre-trained low level policies for navigation with legged locomotion.
%     \item 
%     \item COMPOSING COMPLEX SKILLS BY LEARNING TRANSITION POLICIES~\cite{lee_composing_2019}
%     \item MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies~\cite{peng_mcp_2019}
%     \item  MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies

%     \item Robust Recovery Controller for a Quadrupedal Robot using Deep Reinforcement Learning\cite{lee_robust_2019}
%     \item Modular multitask reinforcement learning with
% policy sketches \cite{andreas_modular_2017}
%     \item The option-critic architecture \cite{bacon_option-critic_2018}
%     \item DIVIDE-AND-CONQUER REINFORCEMENT LEARNING \cite{ghosh_divide-and-conquer_2018}
%     \item distillation - PLAID
%     \item progressive learning? progressive nets?
%     \item FeUdal Networks for Hierarchical Reinforcement Learning Alexander Sasha Vezhnevets \cite{vezhnevets_feudal_2017}
%     \item Terrain-Adaptive Locomotion Skills Using Deep Reinforcement Learning peng: relies on taking an action based on its value, (overestimated)
%     \item bekencamp - value to predict roa of pendulum (overestimated)
% \end{itemize}


% \begin{itemize}
%     \item Composable Controllers for Physics-Based Character Animation~\cite{faloutsos_composable_2001}
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\label{sec:method}

In this section we describe the problem we are solving and our method for training setup policies. 

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=\columnwidth]{images/Fig2.png}}
\hfill
\subfloat[]{\includegraphics[width=\columnwidth]{images/Fig3.png}}
% \hfill
\caption{a) shows the modular pipeline. A terrain classifier selects which module should be utilised, and the torque from the output of the selected module is applied to the robot, returning robot state and depth image. b) Each module is pre-trained on a single terrain type. The target policy has been designed to traverse a specific terrain condition. The setup policy guides the trajectory of the robot from a default walking controller to the target policy, also learning when to switch to the target policy.}
\label{fig:fig2}
% \vspace{-3mm}
\end{figure}

\subsection{Problem Description}
\label{sec:problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We investigate composing controllers for a dynamic platform with narrow or no state overlap between adjacent behaviours. An example of where this occurs \DIFaddbegin \DIFadd{is }\DIFaddend when a bipedal robot performs a jump over a large block. In this scenario, the robot walks up to the block using a walking policy and then performs a jump with a terrain-specific target policy, where the behaviour involves jumping with both feet. Fig~\ref{fig:fig1} shows that the trajectory of the walk policy does not intersect with the trajectory of the target policy, therefore we require an intermediate policy. While it may be possible to improve the robustness of the target policies after they have been trained (i.e. to include states visited by the walk policy), we consider the case where target behaviours and value functions are provided as a black box and are therefore immutable. Our agent has 12 torque controlled actuators, simulated in PyBullet~\cite{coumans_pybullet_2020}.

We select which terrain module to employ using an oracle terrain classifier (Fig~\ref{fig:fig2}a). From a walking policy, we utilise a setup policy that prepares the robot for the target policy (Fig~\ref{fig:fig2}b)). When to switch from the setup policy to the target policy is also a learned output of the setup policy. We first study the traversal of a single difficult terrain artifact that requires walking on a flat surface and performing a jump. We then consider several diverse terrain types (gaps, hurdles, stairs, and stepping stones). The state provided to each policy is $s_t=[rs_t, I_t]$, where $rs_{t}$ is the robot state and $I_t$ is the perception input at time $t$. \DIFaddbegin \DIFadd{The terrain oracle (ground-truth terrain position), simplifies the behaviour switching logic, where terrain type and robot body position (yaw and height) influence the initial detection of the terrain from the depth sensor. 
}\DIFaddend 

\noindent\textbf{Robot state}: \DIFdelbegin \DIFdel{$rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}, s_{right}, s_{left} ]$}\DIFdelend \DIFaddbegin \DIFadd{$rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{body,t}, \omega_{body,t}, \\ \zeta_{body,t}, \psi_{body,t}, h_{body,t}, s_{right}, s_{left} ]$}\DIFaddend , where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot (four Boolean contact points per foot), \DIFdelbegin \DIFdel{$v_{CoM,t}$ and $\omega_{CoM,t}$ }\DIFdelend \DIFaddbegin \DIFadd{$v_{body,t}$ and $\omega_{body,t}$ }\DIFaddend are the linear and angular velocities of the robot body, \DIFdelbegin \DIFdel{$\theta_{CoM,t}$ and $\phi_{CoM,t}$ }\DIFdelend \DIFaddbegin \DIFadd{$\zeta_{body,t}$ and $\psi_{body,t}$ }\DIFaddend are the pitch and roll angles of the robot body and \DIFdelbegin \DIFdel{$h_{CoM,t}$ }\DIFdelend \DIFaddbegin \DIFadd{$h_{body,t}$ }\DIFaddend is the height of the robot from the walking surface. \DIFaddbegin \DIFadd{The sequence of Euler angles used is yaw $>$ pitch $>$ roll. }\DIFaddend $s_{right}$ and $s_{left}$ are Boolean indicators of which foot is in the swing phase, and \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{are }\DIFaddend updated when the current swing foot makes contact with the ground. Robot body rotations are provided as Euler angles. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\noindent\textbf{Perception}: Perception is a depth sensor mounted to the robot base, with a resolution of $[48,48,1]$, and field of view of 60 degrees. Each pixel is a continuous value scaled between $0-1$, measuring a distance between 0.25 and $\SI{2}{\metre}$ from the robot base. The sensor moves with the body in translation and yaw, we provide an artificial gimbal to keep the sensor fixed in roll and pitch. The sensor is pointed at the robot's feet (downwards 60 degrees so the feet are visible) and covers at least two steps in front of the robot~\cite{zaytsev_two_2015}. We reduce the sampling rate of the perception to $\SI{20}{\hertz}$ (reducing computational complexity), where the simulator operates at $\SI{120}{\hertz}$.

\subsection{Deep Reinforcement Learning for Continuous Control}
\label{sec:ppo}

We consider our task to be a Markov Decision Process $\text{MDP}$, defined by tuple $\{\mathcal{S},\mathcal{A}, \mathcal{R}, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in \mathcal{R}$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability \DIFaddbegin \DIFadd{matrix }\DIFaddend from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. 

The goal of reinforcement learning is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. Actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is the joint commands. Each policy is trained with Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. We use the implementation of PPO from OpenAI Baselines~\cite{dhariwal_openai_2017}.

% We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

% We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[-\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse reduce its probability.

% In practice this loss can be noisy, and result in large updates to the policy. Insteasd we use Proximal Policy Optimisation~\cite{schulman_proximal_2017}, which uses a surrogate loss that is clipped, preventing policy updates that are too large. We also use Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}. 


\subsection{Training Setup Policies}
\label{sec:setup}

For each target terrain type we train a setup policy with the purpose of bridging the trajectories of a default walking policy and the behaviour for traversing the upcoming terrain. The algorithm for training each setup policy is shown in Algorithm~\ref{alg:setup}. 

\textbf{Default Policy}: 
The default policy is a pre-trained policy designed to walk on a flat surface. When training a setup policy we always begin with the default policy until the terrain artifact is detected by an oracle. Once the terrain has been traversed, we switch back to the default policy when a termination criteria is reached ($\tau_\theta$, defined below). We initialise the setup policy from the default walking policy such that the robot continues to walk towards the obstacle while learning how to prepare for the target policy.

\textbf{Setup Policy}: 
When terrain type $i$ is detected, we switch immediately from the default policy to the setup policy for terrain type $i$, denoted as $\pi_\phi^i$. While training we are given access to an oracle terrain detector that indicates when the robot is \DIFaddbegin \DIFadd{at }\DIFaddend a fixed distance from the terrain artifact. The setup policy outputs joint torques $a_i$, and switch condition $\tau_\phi$. If the switch condition is met, we immediately switch to the target policy.

\textbf{Target Policy}: 
The target policy for terrain type $i$, denoted as $\pi_\theta^i$, is trained with curriculum learning following the method outlined in prior work~\cite{tidd_guided_2020}. We also define a termination condition $\tau_\theta$ that denotes switching from the target policy back to the default policy. For the \DIFdelbegin \DIFdel{the }\DIFdelend termination condition to be reached, the robot must successfully traverse the terrain obstacle and have both feet in contact with the ground. This condition is the same for all artifact types.
% , and a positive forward velocity $vx$.

\textbf{Setup Policy Reward}: 
We design a reward function to motivate the setup policy to transition the robot from states visited by the default policy to states required by the target policy. We note the value function of the target policy, \DIFdelbegin \DIFdel{$V^{\pi_\theta^i}(s_t) = \sum_{t=0}^{T}\gamma^tr_t$}\DIFdelend \DIFaddbegin \DIFadd{$V^{\pi_\theta^i}(s_t) \approx \sum_{t=0}^{T}\gamma^tr_t$}\DIFaddend , (where $r_t$ is the original reward afforded by the environment \DIFdelbegin \DIFdel{for }\DIFdelend \DIFaddbegin \DIFadd{during training of }\DIFaddend the target policy), provides an estimate of what return \DIFdelbegin \DIFdel{we can expect }\DIFdelend \DIFaddbegin \DIFadd{can be expected }\DIFaddend if we run the target policy \DIFaddbegin \DIFadd{$\pi_\theta^i$ }\DIFaddend from $s_t$. However, value functions are notoriously over-optimistic for states that have not been visited~\cite{haarnoja_soft_2018} (such as those we might experience by running the default policy). \DIFaddbegin \DIFadd{The discrepancy in actual versus expected return is called the }\textit{\DIFadd{advantage}}\DIFadd{. 
}

%DIF >  V^{\pi_\theta^i}(s_t)
%DIF >  V_{theta_V}^{pi_theta^i}
\DIFaddend 

The \DIFdelbegin \DIFdel{advantage }\DIFdelend \DIFaddbegin \textit{\DIFadd{advantage}} \DIFaddend is a zero centered calculation of how much better or worse policy $\pi$ performs \DIFaddbegin \DIFadd{after taking action $a_t$ }\DIFaddend compared to the value function prediction ${V}^\pi(s_t)$:

\begin{equation}
    A^\pi(s_t, a_t) = R_t - V^\pi(s_t)
\end{equation}

where $R_t$ is sum of future rewards from time $t$\DIFaddbegin \DIFadd{, taking action $a_t$, and from there }\DIFaddend running policy $\pi$.

We estimate the advantage using the temporal difference (TD) error with the value function of the target policy $\pi_\theta^i$:

\begin{equation}
    \hat{A}^{\pi_\theta^i}(s_t, a_t) = r_t + \gamma V^{\pi_\theta^i}(s_{t+1}) - V^{\pi_\theta^i}(s_t)
\end{equation}

where $r_t$ is the target policy reward.

Using advantage $\hat{A}^{\pi_\theta^i}(s_t, a_t)$ as an indication of the accuracy of $V^{\pi_\theta^i}(s_t)$, we define the reward \textbf{Advantage Weighted Target Value}:
\begin{equation}
    \hat{r}_t = ( 1 - \text{min}(\alpha\hat{A}^{\pi_\theta^i}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}^{\pi_\theta^i}(s_t)
    \label{eq:eq1}
\end{equation}

where \DIFaddbegin \DIFadd{the target policy value is weighted by the estimated advantage and }\DIFaddend $\alpha$ and $\beta$ are scaling factors tuned empirically (set to 0.15 and 0.01 respectively).

The target policy value function $V^{\pi_\theta^i}(s_t)$ has learned the value for states where the target policy has collected experience. Outside of these states, for example when the robot is activating a different policy, we expect the reward provided by the environment $r_t$, and the next state $s_{t+1}$ will not be consistent with what is expected by the target policy value function. Therefore, the advantage $\hat{A}^{\pi_\theta^i}(s_t, a_t)$ will not be close to zero, and $\hat{r}_t$ becomes small. Intuitively, for states where the target policy value function $V^{\pi_\theta^i}(s_t)$ is accurate, the target policy advantage $\hat{A}^{\pi_\theta^i}$ will be close to zero, thus the setup policy will learn to maximise $V^{\pi_\theta^i}$. \DIFdelbegin \DIFdel{States where $\hat{A}^{\pi_\theta^i}$ }\DIFdelend \DIFaddbegin \DIFadd{State-action pairs where $\hat{A}^{\pi_\theta^i}(s_t, a_t)$ }\DIFaddend is far from zero will reduce the effect of an overconfident \DIFdelbegin \DIFdel{$V^{\pi_\theta^i}$}\DIFdelend \DIFaddbegin \DIFadd{$V^{\pi_\theta^i}(s_t)$}\DIFaddend . 

\textbf{Extended Reward}: 
One issue with training setup policies is the delayed effect of actions, where once switched to the target policy, the setup policy is no longer acting on the environment or receiving a reward. Once the setup policy has transitioned to the target policy, we must provide the setup policy with information regarding the performance of the robot since switching. Our method for solving this problem is to provide the additional reward obtained \textit{after} switching, by including an extended reward in the rollout buffer of the setup policy. We add this extended reward to the last reward received running the setup policy: 
\begin{equation}
    % \text{Buffer}[\hat{r}][-1] \mathrel{+}= \hat{r}_t    
    \hat{r}_{final} = \hat{r}\DIFdelbegin \DIFdel{_{final} }\DIFdelend \DIFaddbegin \DIFadd{_{final\_prev} }\DIFaddend + \hat{r}_t 
\end{equation}
where \DIFdelbegin \DIFdel{$\hat{r}_{final}$ }\DIFdelend \DIFaddbegin \DIFadd{$\hat{r}_{final\_prev}$ }\DIFaddend is the final reward entry received by the setup policy before switching, and $\hat{r_t}$ is the reward received at time $t$, after the setup policy has transitioned to the target policy. For algorithmic stability, we clear all but the last entry of the buffer after each training update. The last reward entry of the buffer becomes $\hat{r}_{final}$ for environment steps that continue after training. The procedure for training setup policies is provided in Algorithm~\ref{alg:setup}. Note that the termination variable $\tau_t$ (line 7) is either $\tau_\phi$ if the current policy is the setup policy, or $\tau_\theta$ if the current policy is the target policy.

\begin{algorithm}
	\caption{Setup Before Switching} 
	\begin{algorithmic}[1]
      \State Load Target Policy $\pi_\theta^i$. Load Default Policy $\pi_\theta^j$
      \State Initialise Setup Policy $\pi_\phi^i$ from the Default Policy
      \State Initialise Buffer
        \State Current Policy $\gets$ Default Policy
		\For {$iteration=1,2,\ldots$}
		    \While {not $done$}
    		    \State $a_t, \tau_t \sim $ Current Policy$(s_t)$ \Comment{$\tau$ is $\tau_\phi$ or $\tau_\theta$}
    		  %  (\tau is either \tau_\phi or \tau_\theta)
    		  %  \State ($\tau = \tau_\theta || \tau_\phi$)
    		    %\Comment{$\tau_\theta$ if Current Policy == }
    		    \State $s_{t+1}, r_t, done = env.step(a_t)$
    		    \If{Terrain detected}
    	            \State $\hat{A}^{\pi_\theta^i}(s_t, a_t) = r_t + \gamma V^{\pi_\theta^i}(s_{t+1}) - V^{\pi_\theta^i}(s_t)$
        		    \State $\hat{r}_t = (1 - \text{min}(\alpha\hat{A}^{\pi_\theta^i}(s_t, a_t)^2, 1))\cdot \beta V^{\pi_\theta^i}(s_t)$
        		    \If{Current Policy == Default Policy}
        		        \State Current Policy $\gets$ Setup Policy $\pi_\phi^i$
        		        \State $\tau_t \gets \tau_\phi$
            		\ElsIf{Current Policy == Setup Policy}
        		        \State Store $s_t$, $a_t$, $\hat{r}_t$, $\tau_\phi$ into Buffer
                        \If{Buffer Full}
                            \State PPO Training Update
                            \State Clear buffer (except last entry)
                        \EndIf
            		    \If {$\tau_\phi$}
            		        \State Current Policy $\gets$ Target Policy $\pi_\theta^i$
            		        \State $\tau_t \gets \tau_\theta$
            		    \EndIf
        			\ElsIf{$\tau_\theta$}
        			    \State Current Policy $\gets$ Default Policy $\pi_\theta^j$
        		    \EndIf
        		    \If{Current Policy != Setup Policy}
        			 %   \State Buffer$[\hat{r}][-1] \mathrel{+}= \hat{r}_t$
        			    \State \DIFdelbegin \DIFdel{$\hat{r}_{final} = \hat{r}_{final} + \hat{r}_t$ 
        			}\DIFdelend \DIFaddbegin \DIFadd{$\hat{r}_{final} = \hat{r}_{final\_prev} + \hat{r}_t$ 
        			}\DIFaddend \EndIf
        		\EndIf
        		\State $s_t = s_{t+1}$
        	\EndWhile
		\EndFor
	\end{algorithmic} 
\label{alg:setup}
\end{algorithm}
% \vspace{15mm}
% \subsection{Terrain Classification}
% \label{sec:classifier}

% Classifier Network \textbf{TBD}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

We evaluate our method with a biped in simulation. Initial evaluations are performed with a single difficult terrain (Sec~\ref{sec:ablation}, Sec~\ref{sec:reward_choice}, Sec~\ref{sec:comparisons}), before adding more behaviours in Sec~\ref{sec:multi_terrain}. The difficult terrain is a sample of flat terrain with a single block 50 cm high, and 30 cm in length (in the forward direction of the robot), an example is shown in Fig.~\ref{fig:fig1}. We perform training and evaluation on a single terrain sample, starting the robot from a random $x$ (forward direction) uniformly sampled from (0.0, 2.2) $\si{\meter}$ before the terrain artifact, $y$ (strafe) uniformly sampled from (-0.6, 0.6) $\si{\meter}$, and $heading$ (yaw) uniformly sampled from (-0.3, 0.3) $\si{\radian}$. \DIFaddbegin \DIFadd{Setup policies are trained for a total of 10 million environment steps collected from 16 worker nodes, each performing a policy update every 2048 steps with averaged gradients. }\DIFaddend All experiments using a single terrain type are evaluated by pausing training and performing 100 evaluation runs, and recording both the Success percentage and Distance percentage. Success \% is defined as the average success rate to reach a goal location several meters past the terrain artifact. Distance \% is the average percentage of total terrain distance the agent successfully covered. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effect of Using Initialisation and Extended Reward}
\label{sec:ablation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We perform an ablation to study the effect of initialising the setup policy from the walking policy, and the effect of extending the reward after the setup policy has transitioned to the target policy. In all experiments the default policy is used until the terrain is detected, then the setup policy is activated until the termination signal $\tau_\phi$ indicates switching to the target policy, and $\tau_\theta$ then results in switching back to the default policy.

\begin{itemize}[leftmargin=*]

\item\textbf{Without Initialisation:} We evaluate our method without initialising the setup policy from the default walking policy, i.e. the setup policy is randomly initialised.

\item\textbf{Without Extended Reward:} We evaluate our method without including the reward after the setup policy has switched to the target policy. 

\item\textbf{Full Method:} Our method uses a setup policy initialised from the default walk policy, and receives reward signal after the setup policy has transitioned to the target policy. 

\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Initialisation        & 38.8      & 73.2  \\
        Without Extended Reward       & 12.3      & 58.3  \\
        Full Method                          & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study for initialising setup policies from a default walk policy, and receiving an extended reward, for switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:results}
\end{table}

We can see that initialising the setup policy with the default walking policy and extending the reward improves learning outcomes as shown in Table~\ref{tab:results}, where our method achieves 82.2\% success compared to 38.8\% without initialisation from the default walking policy and 12.3\% without receiving the extended reward. 
% It is worth noting that training without initialisation from the walking policy required many more training steps to reach an asymptotic result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setup Policy Reward Choice}
\label{sec:reward_choice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For training the setup policy, we investigate several options for the reward provided at each timestep. For each reward type we evaluate with three different random seeds, results are shown in Fig~\ref{fig:results}.

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=\columnwidth]{images/results.png}
\hfill
\caption{We investigate several options for the reward function used to train a setup policy on the difficult jump terrain. We show the success rate (robot reaches several meters after the jump) during training for three different random seeds.}
\label{fig:results}
% \vspace{-3mm}
\end{figure}

\begin{itemize}[leftmargin=*]
\item\textbf{Original:} The reward afforded by the environment that is used to train the target policy: the reward encourages following an expert motion. 

\item\textbf{Constant:} At each timestep a constant reward of 1.5 is given.

\item\textbf{Target Torque:} We encourage the setup policy to match the output of the target policy by minimising the error: $\exp[-2.0\cdot (\pi_\phi(s_t) - \pi_\theta(s_t))^2]$. 

\item\textbf{Target Value:} We evaluate the effect of using the target policy value function as the reward for the setup policy. This is not the same as the original reward, as it is not provided by the environment, but by $\beta V^{\pi_\theta^i}(s_t)$, where $\beta$ is scaling factor 0.01.
%  maximising the target policy value function 

\item\textbf{Advantage Weighted Target Value:} We evaluate the reward introduced in Equation \ref{eq:eq1}.

\end{itemize}

It can be seen from Fig~\ref{fig:results} that a reward using \textbf{Advantage Weighted Target Value} performs better than other reward choices, achieving the highest average success rate (78.7\%). Using the target value reaches a success rate of 63.9\%. This disparity, and the large variation in the target value (green line), shows the effect of over estimation bias often seen with value functions, validating our idea that weighting the value by the advantage reduces the effect of this bias when training setup policies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparisons}
\label{sec:comparisons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We compare our method with several others, including end to end methods, without using setup policies, and a method that uses proximity prediction to train a transition policy~\cite{lee_composing_2019}.

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success\% & Distance\% \\
       \hline
        Single Policy                 & 0.0           & 11.3  \\
        Single Policy With Curriculum & 0.0           &  3.8 \\
        \DIFdelbeginFL \DIFdelFL{No Setup Policy               }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{Without Setup Policies              }\DIFaddendFL & 1.5           & 51.3 \\
        Learn When to Switch          & 0.0           & 44.2  \\
        Proximity Prediction         & 51.3           & 82.4 \\
        Setup Policy (Ours)         & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success and average distance of the total length covered when switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:results_compare}
\end{table}

\begin{itemize}[leftmargin=*]

\begin{figure*}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth]{images/Fig1_2.png}
\includegraphics[width=\textwidth]{images/all.png}
\hfill
\caption{Setup policies enable a biped to transition between complex visuo-motor behaviours for traversing a sequence of diverse terrains.}
\label{fig:multi}
% \vspace{-3mm}
\end{figure*}

\item\textbf{Single Policy:} We train a single end to end policy on the terrain sample.

\item\textbf{Single Policy With Curriculum:} We utilise curriculum learning to train a single end to end policy on the terrain sample (using the method outlined in~\cite{tidd_guided_2020}).

\item\textbf{\DIFdelbegin \DIFdel{No }\DIFdelend \DIFaddbegin \DIFadd{Without }\DIFaddend Setup \DIFdelbegin \DIFdel{Policy}\DIFdelend \DIFaddbegin \DIFadd{Policies}\DIFaddend :} We switch to the target policy from the default policy as soon as the terrain oracle detects the next terrain.

\item\textbf{Learn When to Switch:} We collect data by switching from the default policy to the target policy at random distances from the Jump. We use supervised learning to learn when the robot is in a suitable state to switch. Details of this method is found in our previous work~\cite{tidd_learning_2021}.

\item\textbf{Proximity Prediction:} We follow the method defined by Lee et al.~\cite{lee_composing_2019} to train Transition Policies (one for each behaviour) using a proximity predictor function $P(s_t)$. $P(s_t)$ outputs a continuous value that indicates how close the agent is to a configuration that resulted in successful traversal. $P(s_t)$ is trained using supervised learning from success and failure buffers. The reward used to train the transition policy is the dense reward created by  $P(s_{t+1}) - P(s_{t})$, encouraging the agent to move closer to a configuration that results in successful switching. For accurate comparison we initialise the transition policy with weights from the walk policy, and utilise the terrain oracle for policy selection (the paper refers to a rule-based meta-policy in place of a terrain oracle~\cite{lee_composing_2019}).

\item\textbf{Setup Policy (Ours):} We follow Algorithm~\ref{alg:setup} to train setup policies. 

\end{itemize}

We can see from Table~\ref{tab:results_compare} that our method for developing setup policies performs the best (82.2\% success rate), compared to other methods. A single policy was unable to traverse the difficult jump terrain, even with an extended learning time and curriculum learning. The poor performance of \textbf{Single Policy With Curriculum} was the result of the robot not progressing through the curriculum, and as a consequence is unable to move without assistive forces \DIFaddbegin \DIFadd{during evaluation. In contrast, the single policy trains without assistive forces, so while the single policy still fails to complete the task, it is able to make forward progress when evaluated. These results highlight the difficulty of learning to walk and jump as a single behaviour}\DIFaddend . We show that setup policies are necessary for this problem, with \textbf{\DIFdelbegin \DIFdel{No }\DIFdelend \DIFaddbegin \DIFadd{Without }\DIFaddend Setup \DIFdelbegin \DIFdel{Policy}\DIFdelend \DIFaddbegin \DIFadd{Policies}\DIFaddend } unable to successfully traverse the terrain (1.5\% success). \textbf{Learning When to Switch} also performed poorly as there are very few states that overlap between the default policy and the target policy for the switch estimator to learn. The \textbf{Proximity Prediction} method was able to successfully traverse the jump 51.3\% of the time. It is worth noting that this method required approximately three times more training episodes than our method to reach the provided results, despite also being initialised from the default policy.

%DIF >  The poor performance of \textbf{Single Policy With Curriculum} was the result of the robot not progressing through the curriculum, and as a consequence is unable to move without assistive forces.
\DIFaddbegin 

\DIFaddend These experiments show that for the difficult jump terrain, we require a specialised target policy dedicated to learning the complex jumping behaviour. We show that this specialised policy has a trajectory that does not overlap with the default policy, and thus setup policies are required. Our method for learning \DIFdelbegin \DIFdel{a }\DIFdelend setup policies achieved the highest performance on this difficult task.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Multiple Terrain Types}
\label{sec:multi_terrain}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


For our final experiment we train setup policies for several additional terrain types. In total we now have modules for jumps, gaps, hurdles, stairs, and stepping stones. Fig~\ref{fig:multi} shows a sequence with each terrain type. We follow the pipeline shown in Fig~\ref{fig:fig2}a), where a terrain oracle determines which module should be selected. On selection, the setup policy is employed until the robot reaches a switch state ($\tau_\phi$), then switching to the target policy.
Termination criteria $\tau_\theta$ (introduced in Sec~\ref{sec:method}) determines when to switch back to the default policy for the jump obstacle only. All other policies resemble the behaviour of the default policy on flat terrain, i.e. we continue using the target policy after the terrain has been traversed for gaps, hurdles, stairs, and stepping stones, until the oracle determines the terrain has changed.

We evaluate with a sequence of each of the 5 terrain types, randomly shuffled before each run. We perform 1000 runs, with a total of 5000 various terrain types to be traversed. In Table~\ref{tab:multi_results} we show the average percentage of total distance travelled and success rate with and without using setup policies. A successful run in this scenario is defined as traversing the last terrain in the sequence. Table~\ref{tab:multi_breakdown} shows the failure count for each terrain type.
% Table~\ref{tab:multi_breakdown} shows the individual performance of the agent for each terrain type (number of successful traversals / total traversals).

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Setup Policies        & 1.9      & 36.3  \\
        % With setup policies       & \textbf{26.4}      & \textbf{53.2}  \\
        With Setup Policies       & \textbf{71.2}      & \textbf{80.2}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success rate and percentage of the total terrain length travelled from 1000 episodes of all 5 terrain types, randomly shuffled each episode.}
    \label{tab:multi_results}
\end{table}

\begin{table}[h!]
    \DIFdelbeginFL %DIFDELCMD < \vspace{-2mm}
%DIFDELCMD <     %%%
\DIFdelendFL \DIFaddbeginFL \vspace{-9mm}
    \DIFaddendFL \centering
    \begin{adjustbox}{min width=0.9\columnwidth}
    \begin{tabular}{cccccc}
                                      & Jump & Gap & Hurdle & Stairs & Steps \\
      \hline
        % Without setup policies       & 710      & 90  & \textbf{43} &  \textbf{20} & \textbf{90}  \\
        Without Setup Policies       & 782      & 52  & \textbf{36} &  \textbf{31} & \textbf{86}  \\
        % With setup policies        & \textbf{420}      & \textbf{70}  & 73 & 36 & 144 \\
        With Setup Policies        & \textbf{36}      & \textbf{48}  & 43 & 65 & 96 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Number of failures by terrain type from 1000 episodes of all 5 terrain types, randomly shuffled each episode.}
    \label{tab:multi_breakdown}
\end{table}

\begin{table}[h!]
    \DIFdelbeginFL %DIFDELCMD < \vspace{-2mm}
%DIFDELCMD <     %%%
\DIFdelendFL \DIFaddbeginFL \vspace{-9mm}
    \DIFaddendFL \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Setup Policies        & 68.2      & 78.1  \\
        With Setup Policies       & \textbf{76.7}      & \textbf{84.6}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success rate and percentage of the total terrain length travelled from 1000 episodes of 4 terrain types \textbf{(without the jump terrain)}, randomly shuffled each episode}
    \label{tab:multi_results_no_jumps}
\end{table}

\begin{table}[h!]
    \DIFdelbeginFL %DIFDELCMD < \vspace{-2mm}
%DIFDELCMD <     %%%
\DIFdelendFL \DIFaddbeginFL \vspace{-9mm}
    \DIFaddendFL \centering
    \begin{adjustbox}{min width=0.82\columnwidth}
    \begin{tabular}{ccccc}
                                      & Gap & Hurdle & Stairs & Steps \\
      \hline
        Without Setup Policies       & 74  & \textbf{41} &  64 & 142  \\
        With Setup Policies        &  \textbf{44}  & 51 & \textbf{49} & \textbf{90} \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Number of failures by terrain type from 1000 episodes of 4 terrain types \textbf{(without the jump terrain)}, randomly shuffled each episode.}
    \label{tab:multi_breakdown_no_jumps}
\end{table}
\DIFdelbegin %DIFDELCMD < \newpage
%DIFDELCMD < %%%
\DIFdelend %DIF >  \newpage
%DIF >  \newline
\DIFaddbegin \vspace{-6mm}
\DIFaddend We can see from Table~\ref{tab:multi_results} that setup policies improve the success rate compared to switching policies without the intermediate policy (71.2\% success compared to 1.9\%). Table~\ref{tab:multi_breakdown} provides a breakdown of the number of times the robot failed on each terrain. From Table~\ref{tab:multi_breakdown} we can see that setup policies are most critical for traversing the difficult jump terrain (reducing the failures from 782 to 36), though we also see improvements for gap terrain. 

\DIFaddbegin \vspace{2.5mm}
\DIFaddend To investigate further, we exclude the jump obstacle from the terrain sequence and still observe a significant benefit using setup policies. Table~\ref{tab:multi_results_no_jumps} shows the performance increase from 68.2\% to 76.7\% of successful traversals for 4 terrain types (excluding the jump obstacle). \DIFdelbegin \DIFdel{The }\DIFdelend \DIFaddbegin \DIFadd{Common failure modes were seen when the robot veered from the walking line (centre y position) and was unable to recover in time for the next upcoming terrain. This often occurred before the }\DIFaddend stepping stone obstacle\DIFaddbegin \DIFadd{, which }\DIFaddend had the highest failure rate of the remaining terrain types \DIFdelbegin \DIFdel{, investigation is required to improve the setup policies for this terrain (Table ~}\DIFdelend \DIFaddbegin \DIFadd{(Table~\ref{tab:multi_breakdown_no_jumps}). Setup policies showed a clear benefit for each separate terrain type, however, we can see with the multi-terrain experiments there were cases where not using setup policies performed better (Table \ref{tab:multi_breakdown} and }\DIFaddend \ref{tab:multi_breakdown_no_jumps}). \DIFaddbegin \DIFadd{For the behaviours that did not require jumping with both feet switching early (}\textbf{\DIFadd{Without Setup Policies}}\DIFadd{) gave the robot time to correct its walking line before approaching the next terrain. 
}\DIFaddend 

\DIFaddbegin \vspace{2.5mm}
\DIFaddend Despite the clear need for setup policies, we attribute failures to out of distribution states, i.e. the robot visits states in the terrain sequence that it does not experience when training \DIFdelbegin \DIFdel{the setup policy }\DIFdelend on the individual terrain types. \DIFaddbegin \DIFadd{Earlier implementations found that training setup policies from less diverse starting locations resulted in poor performance when evaluated across multiple terrain types. In these experiments, setup policies successfully guided the robot during a set stage of the walking cycle, however were unable to control the robot when in other stages of walking, as were common after traversing different terrain types. }\DIFaddend Training setup policies for \DIFaddbegin \DIFadd{a }\DIFaddend wider range of states will be investigated in future work. 
\DIFdelbegin \DIFdel{Furthermore, the performance of behaviours on each individual terrain type could be analysed to improve the generalisation of this method to new behaviours.
}\DIFdelend \DIFaddbegin 

%DIF >  Furthermore, the performance of behaviours on each individual terrain type could be analysed to improve the generalisation of this method to new behaviours.

%DIF >  investigation is required to improve the setup policies for this terrain (Table~\ref{tab:multi_breakdown_no_jumps}).
\DIFaddend 


% While the results show that without setup policies the hurdle, stairs, and steps terrain appear to have less failures than running setup policies, we note that these terrains are visited far less times when running without setup policies due to significant failure with the jumps terrain.

% These results show the highest failure rate on the multi terrain setup is on the jump terrain, and that there is clear room for improvement on this terrain. 


%  For example, if the robot was on a gap, and using the gaps behaviour, then switches to the jumps setup policy to prepare for an upcoming jump, it will not necessarily be in a state that has been seen during training.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

It is common practice for legged robots to have separate locomotion policies to traverse different terrain conditions. We propose setup policies that enable smooth transition from the trajectory of one locomotion policy to the trajectory of a target policy for traversing difficult terrain with a dynamic biped. We use deep reinforcement learning to learn the setup policies for which we introduce a novel reward based on the Advantage Weighted Target Value, utilising the scaled value prediction of the target policy as the reward for the setup policy. 

In simulation experiments for transitioning from a walking policy to a jumping policy, we show using an in-between setup policy yields a higher success rate compared to using a single policy (0$\%$ success rate), or the two policies without the setup policy (from 1.5$\%$ success rate without setup policies to 82$\%$). We further show that our method is scalable to other terrain types, and demonstrate the effectiveness of the approach on a sequence of difficult terrain conditions, improving the success rate from 1.9$\%$ without setup policies to 71.2$\%$.

A limitation of our method is that setup policies are trained from a default walking policy. We would like to improve the scope of the setup policies such that a wider range of states are funnelled towards the target policy. \DIFdelbegin \DIFdel{If we allowed further training of the target policies, our training method could be used to include more states and improve robustness. }\DIFdelend The idea of utilising the advantage (estimated by the temporal difference (TD) error) as a confidence metric can be applied generally for region of attraction (RoA) expansion, safe reinforcement learning, and also for blending several behaviours for performing complex composite tasks. These ideas will be explored in future work. A significant assumption in this work is that we have access to a terrain oracle, removing this dependency will \DIFaddbegin \DIFadd{be }\DIFaddend required as we consider experiments in the real world.

%DIF >  If we allowed further training of the target policies, our training method could be used to include more states and improve robustness. 
\DIFaddbegin 

\DIFaddend %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DIFaddbegin 


\DIFaddend % balance the last page
\addtolength{\textheight}{-2cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.
% might need that \newpage
\bibliographystyle{IEEEtran}
\bibliography{references}
\end{document}



==> main.tex <==

\begin{document}

\title{\LARGE \bf
Learning Setup Policies: Reliable Transition
\\ Between Locomotion Behaviours}

\author{Brendan Tidd$^{1,2}$, Nicolas Hudson$^{3}$, Akansel Cosgun$^{4}$ and J\"{u}rgen Leitner$^{5,6}$%
\thanks{Manuscript received: March, 13th, 2022; Revised July, 27th, 2022; Accepted August, 25th, 2022.}%Use only for final RAL version
\thanks{This paper was recommended for publication by
Editor Abderrahmane Kheddar upon evaluation of the Associate Editor and
Reviewers’ comments.} %Use only for final RAL version

\thanks{$^{1}$Queensland University of Technology (QUT), Australia}%
\thanks{$^{2}$Robotics and Autonomous Systems Group, CSIRO, Pullenvale, QLD 4069, Australia
{\tt\footnotesize brendan.tidd@data61.csiro.au}}
% \newline Email: brendan.tidd@data61.csiro.au}
\thanks{$^{3}$Amazon Robotics AI, USA}%
\thanks{$^{4}$Deakin University, Australia}%
\thanks{$^{5}$Monash University, Australia}%
\thanks{$^{6}$LYRO Robotics Pty Ltd, Australia}%
%\thanks{$^{4}$Australian Centre for Robotic Vision}%

% \thanks{$^{1}$First Author and Third Author are with School of Engineering, Robotics Department, University of Somewhere, Someland
%         {\tt\footnotesize first.author@papercept.net}}%
% \thanks{$^{2} $SecondAuthor is with School of Engineering, Automation Department, University of Anywhere, Anyland
%         {\tt\footnotesizel second.author@papercept.net}}%
\thanks{Digital Object Identifier (DOI): see top of this page.}
}

\markboth{IEEE Robotics and Automation Letters. Preprint Version. Accepted September, 2022}
{Tidd \MakeLowercase{\textit{et al.}}: Learning Setup Policies: Reliable Transition Between Locomotion Behaviours} 


\maketitle
% \thispagestyle{empty}
% \pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
\label{sec:abstract}
Dynamic platforms that operate over many unique terrain conditions typically require many behaviours. To transition safely, there must be an overlap of states between adjacent controllers. We develop a novel method for training setup policies that bridge the trajectories between pre-trained Deep Reinforcement Learning (DRL) policies. We demonstrate our method with a simulated biped traversing a difficult jump terrain, where a single policy fails to learn the task, and switching between pre-trained policies without setup policies also fails. We perform an ablation of key components of our system, and show that our method outperforms others that learn transition policies. We demonstrate our method with several difficult and diverse terrain types, and show that we can use setup policies as part of a modular control suite to successfully traverse a sequence of complex terrains. We show that using setup policies improves the success rate for traversing a single difficult jump terrain (from 51.3$\%$ success rate with the best comparative method to 82.2$\%$), and traversing a random sequence of difficult obstacles (from 1.9$\%$ without setup policies to 71.2$\%$).


% \textbf{why do I care?}
% , as it may not be possible to safely switch between controllers outside of the overlapping states.
\end{abstract}

\begin{IEEEkeywords}
Humanoid and bipedal locomotion, reinforcement learning, vision-based navigation.
\end{IEEEkeywords}
\IEEEpeerreviewmaketitle

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:introduction}

\IEEEPARstart{B}{ipedal} robots have the capability to cover a span of terrains that humans can traverse. This makes bipeds an appealing locomotion option for robots in human environments. It is impractical, however, to design a single controller that works over all required environments, particularly if all conditions are not known a priori. For robots to be able to perform a number of diverse behaviours, it is desirable for a control suite to be modular, where any number of behaviours can be added with minimal retraining.

% included in the control repertoire. 
% Ideally, as new conditions are identified and new controllers become available, the new behaviours can be added to the control suite with minimal retraining.
 
Deep Reinforcement Learning (DRL) is an appealing method for developing visuo-motor behaviours for legged platforms. However, such DRL policies are usually trained on the terrain they are expected to operate, though it is unlikely that the agent would have access to a complete set of terrain conditions during policy training before deployment. Controllers for dynamic platforms are typically developed and tuned with safety harnesses and human supervisors in order to minimise potential damage to the robot and the environment. These restrictions limit the development of controllers over an exhaustive collection of terrain conditions. Furthermore, modifying controllers that have already been tuned is costly, for example DRL methods that are trained for discrete terrain types typically require retraining if new terrain variations are introduced \cite{peng_dynamic_2015}. We propose training a \textit{setup policy} to transition between two pre-trained policies targeting different terrains.

A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over if controllers are switched when the robot is not in a safe region for the subsequent controller. Figure~\ref{fig:fig1} shows our primary contribution: a setup policy that prepares the robot for the necessary controller to traverse the upcoming terrain obstacle. With our method, we can transition between existing behaviours, allowing pre-trained DRL policies to be combined. 

% We propose a modular approach to developing a control suite for a biped expected to traverse a number of difficult terrain artifacts, where all terrain conditions are not known when training each module. A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over. Figure~\ref{fig:fig1} shows our primary contribution: a setup policy that prepares the robot for the upcoming terrain artifact. With our method, we can safely transition between behaviours that are developed separately, such that any number of pre-trained DRL policies can be combined, without any re-training of low level policies.  

\begin{figure}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth,natwidth=610,natheight=642]{images/Fig1.png}
\includegraphics[width=\columnwidth]{images/Fig1.png}
% \includegraphics[width=\columnwidth]{images/Fig1_err.png}
\hfill
\caption{As the robot approaches a difficult terrain artifact, it must move into position for target policy $i$. The trajectory of the walking policy $j$ (shown with a blue line), does not intersect with the trajectory of the target policy $i$ (green line). Our setup policy provides a trajectory that prepares the robot for the upcoming target policy (orange line).}
\label{fig:fig1}
\vspace{-3mm}
\end{figure}
% How can we leverage subpolicy learning to improve learning outcomes?
Our contributions are as follows:
\begin{itemize}
    \item Using pre-trained policies, we develop \textbf{setup policies} that significantly improve the success rate from transitioning from a default walking policy to a target policy. The setup policy also learns when to switch to the target policy. 
    \item We introduce a novel reward, called \textbf{Advantage Weighted Target Value}, guiding the robot towards the target policy.
    \item We show that we can use setup policies with several difficult terrain types, allowing for a modular control suite, combining behaviours that have been trained separately without any retraining of low level policies.
\end{itemize}

% The organization of this paper is as follows. After reviewing the relevant literature in Sec~\ref{sec:related_work}, we define the problem in Sec~\ref{sec:problem}, the learning algorithm in Sec~\ref{sec:ppo}, and our method for developing setup policies in Sec~\ref{sec:setup}. Our experimental results and comparisons are shown in Sec~\ref{sec:experiments}. Finally, we conclude with a brief discussion in Sec~\ref{sec:conclusion}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:related_work}
% Related work should also be story, starting from the start of the problem, highlighting what is missing, and refining to the specific paper that is closest to ours. Goal is to find gaps, start broad, and funnel into specifics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Deep reinforcement learning (DRL) has demonstrated impressive results for locomotion tasks in recent works~\cite{heess_emergence_2017, peng_deeploco_2017, peng_deepmimic_2018, xie_allsteps_2020}. Typically DRL policies optimise a single reward function, as new environments and behaviours are introduced costly retraining is required. Single policies have demonstrated locomotion over various terrains for simple 2D cases \cite{song_recurrent_2018}, and impressive quadruped behaviours \cite{lee_learning_2020, rudin_learning_2021}, however, for many scenarios multiple policies are often required. Furthermore, developing a single policy to perform multiple behaviours can degrade the performance of each behaviour~\cite{lee_robust_2019}.

Hierarchical reinforcement learning (HRL) offers flexibility through architecture, by training all segments of the hierarchy concurrently~\cite{sutton_between_1999, bacon_option-critic_2018, frans_meta_2018,peng_deeploco_2017}, or training parts of the hierarchy separately~\cite{merel_hierarchical_2019},~\cite{lee_composing_2019}.  When trained together, HRL can improve task level outcomes, such as steering and object tracking~\cite{peng_deeploco_2017}, or improve learning efficiency by reusing low level skills across multiple high level tasks~\cite{frans_meta_2018}. When trained separately, low level controllers can be refined efficiently using prior knowledge, such as by utilising motion capture data~\cite{peng_deepmimic_2018, merel_hierarchical_2019, peng_mcp_2019} or behavioural cloning~\cite{strudel_learning_2020}. For robotics applications it may be difficult to develop controllers for multiple behaviours simultaneously. Using pre-trained primitives can break up a large difficult problem into smaller solvable sub-problems~\cite{schaal_dynamic_2006}.

Using pre-trained policies requires suitable handling of transitions between behaviours. Faloutsos et al.~\cite{faloutsos_composable_2001} learn pre and post-conditions for each controller, such that switching only occurs when these conditions have been satisfied. DeepMimic by Peng et al.~\cite{peng_deepmimic_2018} combines pre-trained behaviours learned from motion capture, with reliance on a phase variable to determine when one behaviour has been completed. Policy sketches introduce a hierarchical method that uses task specific policies, with each task performed in sequence~\cite{andreas_modular_2017}. CompILE uses soft boundaries between task segments~\cite{kipf_compile_2019}. Work by Peng et al.~\cite{peng_terrain-adaptive_2016} trains several actor-critic control policies, modulated by the highest critic value in a given state. For these examples there must be a reasonable state overlap between controllers.

Other methods that combine pre-trained behaviours learn latent representations of skills~\cite{pertsch_accelerating_2020} or primitives~\cite{ha_distilling_2020}, enabling interpolation in the latent space. From an offline dataset of experience, Pertsch et al.~\cite{pertsch_accelerating_2020} were able to combine low level controllers in manipulation tasks and locomotion for a multi-legged agent. In our previous work~\cite{tidd_learning_2021}, we learn when to switch between low level primitives for a simulated biped using data collected by randomly switching between behaviours. Ha et al.~\cite{ha_distilling_2020} utilise motion capture to learn latent representations of primitives, then use model predictive control to navigate with a high dimensional humanoid. The FeUdal approach learns a master policy that modulates
low-level policies using a learned goal signal~\cite{vezhnevets_feudal_2017}. Interpolation between behaviours yields natural transitions~\cite{xu_hierarchical_2020}. The work by Peng et al.~\cite{peng_mcp_2019} combines pre-trained policies using a gating function that learns a multiplicative combination of behaviours to generate smooth actions. Yang et al.~\cite{yang_multi_2020} learn a gating neural network to blend several separate expert neural network policies to perform trotting, steering, and fall recovery in real-world experiments with a quadruped. Da et al.~\cite{da_supervised_2017} use supervised learning to train a control policy for a biped from several manually derived controllers to perform periodic and transitional gaits on flat and sloped ground. In each of these approaches, experience from all behaviours must be available during training. 

For dynamic platforms, where separate controllers occupy different subsets of the state, changing behaviours may result in instability if there is no overlap between controllers. Lee et al.~\cite{lee_composing_2019} learn a proximity predictor to train a transition policy to guide an agent to the initial state required by the next controller. Locomotion experiments are demonstrated with a 2D planar walker, where learning occurs by training with all terrain conditions. We show that our method performs more reliably (with a higher success rate), despite training with experience from a single terrain type. Our setup policies learn to transition between complex behaviours with a 3D biped in a simulation environment using a depth image to perceive the terrain. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Berkencamp, and mace use values to estimate when to use controllers.
% Composing paper. Something more specific about our method: advantage weighted value, this is a primary contribution. Training on sample only. Scaling to any number of policies, only needing data to train classifier, (no training of policies on anything but samples).


% sequential decision making tasks
% with greater sample efficiency than their non-hierarchical counterparts because hierarchical agents can break down tasks into sets of subtasks that only require short
% sequences of decisions.LEARNING MULTI-LEVEL HIERARCHIES WITH
% HINDSIGHT Andrew Levy , Hierarchical Actor-Critic (HAC), . Yet, learning multiple
% levels of policies in parallel is hard because it is inherently unstable: changes in
% a policy at one level of the hierarchy may cause changes in the transition and reward functions at higher levels in the hierarchy, making it difficult to jointly learn
% multiple levels of policies.  The main idea behind HAC is to train each level of the
% hierarchy independently of the lower levels by training each level as if the lower
% level policies are already optimal.

% HIRO Data-Efficient Hierarchical Reinforcement Learning Ofir Nachum - Use reward relabeling - High level give goals to low level. rewards from the environment are reused, temporal abstraction, off-policy.


% The first category lets a high-level policy select a low-level skill to execute [13, 14, 15, 28],
% which we refer to as the selector methods. In the second category, a subgoal is set for the low level by
% high-level policies [8, 9, 11, 10, 25], which we refer to as subgoal-based methods.

% % \subsection{Hierarchical RL}

% % \subsection{Transition Policies and Modular RL}
% % \textbf{ TODO Transition papers
% \begin{itemize}
%     \item sutton \cite{Sutton2017ReinforcementA.G.}
%     \item HRL \cite{sutton_between_1999} - introduces options, a framework for splitting mdp into temporally abstracted options.
%     \item m, HRL with Advantage function-based Auxiliary Rewards \cite{li et al} - Use the advantage of the high level policy as dense reward signal for an otherwise sparse reward problem,  improving pre-trained low level policies for navigation with legged locomotion.
%     \item 
%     \item COMPOSING COMPLEX SKILLS BY LEARNING TRANSITION POLICIES~\cite{lee_composing_2019}
%     \item MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies~\cite{peng_mcp_2019}
%     \item  MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies

%     \item Robust Recovery Controller for a Quadrupedal Robot using Deep Reinforcement Learning\cite{lee_robust_2019}
%     \item Modular multitask reinforcement learning with
% policy sketches \cite{andreas_modular_2017}
%     \item The option-critic architecture \cite{bacon_option-critic_2018}
%     \item DIVIDE-AND-CONQUER REINFORCEMENT LEARNING \cite{ghosh_divide-and-conquer_2018}
%     \item distillation - PLAID
%     \item progressive learning? progressive nets?
%     \item FeUdal Networks for Hierarchical Reinforcement Learning Alexander Sasha Vezhnevets \cite{vezhnevets_feudal_2017}
%     \item Terrain-Adaptive Locomotion Skills Using Deep Reinforcement Learning peng: relies on taking an action based on its value, (overestimated)
%     \item bekencamp - value to predict roa of pendulum (overestimated)
% \end{itemize}


% \begin{itemize}
%     \item Composable Controllers for Physics-Based Character Animation~\cite{faloutsos_composable_2001}
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\label{sec:method}

In this section we describe the problem we are solving and our method for training setup policies. 

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=\columnwidth]{images/Fig2.png}}
\hfill
\subfloat[]{\includegraphics[width=\columnwidth]{images/Fig3.png}}
% \hfill
\caption{a) shows the modular pipeline. A terrain classifier selects which module should be utilised, and the torque from the output of the selected module is applied to the robot, returning robot state and depth image. b) Each module is pre-trained on a single terrain type. The target policy has been designed to traverse a specific terrain condition. The setup policy guides the trajectory of the robot from a default walking controller to the target policy, also learning when to switch to the target policy.}
\label{fig:fig2}
% \vspace{-3mm}
\end{figure}

\subsection{Problem Description}
\label{sec:problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We investigate composing controllers for a dynamic platform with narrow or no state overlap between adjacent behaviours. An example of where this occurs is when a bipedal robot performs a jump over a large block. In this scenario, the robot walks up to the block using a walking policy and then performs a jump with a terrain-specific target policy, where the behaviour involves jumping with both feet. Fig~\ref{fig:fig1} shows that the trajectory of the walk policy does not intersect with the trajectory of the target policy, therefore we require an intermediate policy. While it may be possible to improve the robustness of the target policies after they have been trained (i.e. to include states visited by the walk policy), we consider the case where target behaviours and value functions are provided as a black box and are therefore immutable. Our agent has 12 torque controlled actuators, simulated in PyBullet~\cite{coumans_pybullet_2020}.

We select which terrain module to employ using an oracle terrain classifier (Fig~\ref{fig:fig2}a). From a walking policy, we utilise a setup policy that prepares the robot for the target policy (Fig~\ref{fig:fig2}b)). When to switch from the setup policy to the target policy is also a learned output of the setup policy. We first study the traversal of a single difficult terrain artifact that requires walking on a flat surface and performing a jump. We then consider several diverse terrain types (gaps, hurdles, stairs, and stepping stones). The state provided to each policy is $s_t=[rs_t, I_t]$, where $rs_{t}$ is the robot state and $I_t$ is the perception input at time $t$. The terrain oracle (ground-truth terrain position), simplifies the behaviour switching logic, where terrain type and robot body position (yaw and height) influence the initial detection of the terrain from the depth sensor. 

\noindent\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{body,t}, \omega_{body,t}, \\ \zeta_{body,t}, \psi_{body,t}, h_{body,t}, s_{right}, s_{left} ]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot (four Boolean contact points per foot), $v_{body,t}$ and $\omega_{body,t}$ are the linear and angular velocities of the robot body, $\zeta_{body,t}$ and $\psi_{body,t}$ are the pitch and roll angles of the robot body and $h_{body,t}$ is the height of the robot from the walking surface. The sequence of Euler angles used is yaw $>$ pitch $>$ roll. $s_{right}$ and $s_{left}$ are Boolean indicators of which foot is in the swing phase, and are updated when the current swing foot makes contact with the ground. Robot body rotations are provided as Euler angles. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\noindent\textbf{Perception}: Perception is a depth sensor mounted to the robot base, with a resolution of $[48,48,1]$, and field of view of 60 degrees. Each pixel is a continuous value scaled between $0-1$, measuring a distance between 0.25 and $\SI{2}{\metre}$ from the robot base. The sensor moves with the body in translation and yaw, we provide an artificial gimbal to keep the sensor fixed in roll and pitch. The sensor is pointed at the robot's feet (downwards 60 degrees so the feet are visible) and covers at least two steps in front of the robot~\cite{zaytsev_two_2015}. We reduce the sampling rate of the perception to $\SI{20}{\hertz}$ (reducing computational complexity), where the simulator operates at $\SI{120}{\hertz}$.

\subsection{Deep Reinforcement Learning for Continuous Control}
\label{sec:ppo}
 
We consider our task to be a Markov Decision Process $\text{MDP}$, defined by tuple $\{\mathcal{S},\mathcal{A}, \mathcal{R}, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in \mathcal{R}$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability matrix from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. 

The goal of reinforcement learning is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. Actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is the joint commands. Each policy is trained with Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. We use the implementation of PPO from OpenAI Baselines~\cite{dhariwal_openai_2017}.

% We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

% We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[-\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse reduce its probability.

% In practice this loss can be noisy, and result in large updates to the policy. Insteasd we use Proximal Policy Optimisation~\cite{schulman_proximal_2017}, which uses a surrogate loss that is clipped, preventing policy updates that are too large. We also use Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}. 


\subsection{Training Setup Policies}
\label{sec:setup}

For each target terrain type we train a setup policy with the purpose of bridging the trajectories of a default walking policy and the behaviour for traversing the upcoming terrain. The algorithm for training each setup policy is shown in Algorithm~\ref{alg:setup}. 

\textbf{Default Policy}: 
The default policy is a pre-trained policy designed to walk on a flat surface. When training a setup policy we always begin with the default policy until the terrain artifact is detected by an oracle. Once the terrain has been traversed, we switch back to the default policy when a termination criteria is reached ($\tau_\theta$, defined below). We initialise the setup policy from the default walking policy such that the robot continues to walk towards the obstacle while learning how to prepare for the target policy.

\textbf{Setup Policy}: 
While training setup policies, we are given access to an oracle terrain detector that indicates when the robot is at a fixed distance from the terrain artifact. When terrain type $i$ is detected, we switch immediately from the default policy to the setup policy for terrain type $i$, denoted as $\pi_\phi^i$. The setup policy outputs joint torques $a_i$, and switch condition $\tau_\phi$. If the switch condition is met, we immediately switch to the target policy.

\textbf{Target Policy}: 
The target policy for terrain type $i$, denoted as $\pi_\theta^i$, is trained with curriculum learning following the method outlined in prior work~\cite{tidd_guided_2020}. We also define a termination condition $\tau_\theta$ that denotes switching from the target policy back to the default policy. For the termination condition to be reached, the robot must successfully traverse the terrain obstacle and have both feet in contact with the ground. This condition is the same for all artifact types.
% , and a positive forward velocity $vx$.

\textbf{Setup Policy Reward}: 
We design a reward function to motivate the setup policy to transition the robot from states visited by the default policy to states required by the target policy. We note the value function of the target policy, $V^{\pi_\theta^i}(s_t) \approx \sum_{t=0}^{T}\gamma^tr_t$, (where $r_t$ is the original reward afforded by the environment during training of the target policy), provides an estimate of what return can be expected if we run the target policy $\pi_\theta^i$ from $s_t$. However, value functions are notoriously over-optimistic for states that have not been visited~\cite{haarnoja_soft_2018} (such as those we might experience by running the default policy). The discrepancy in actual versus expected return is called the \textit{advantage}. 

% V^{\pi_\theta^i}(s_t)
% V_{theta_V}^{pi_theta^i}

The \textit{advantage} is a zero centered calculation of how much better or worse policy $\pi$ performs after taking action $a_t$ compared to the value function prediction ${V}^\pi(s_t)$:

\begin{equation}
    A^\pi(s_t, a_t) = R_t - V^\pi(s_t)
\end{equation}

where $R_t$ is sum of future rewards from time $t$, taking action $a_t$, and from there running policy $\pi$.

We estimate the advantage using the temporal difference (TD) error with the value function of the target policy $\pi_\theta^i$:

\begin{equation}
    \hat{A}^{\pi_\theta^i}(s_t, a_t) = r_t + \gamma V^{\pi_\theta^i}(s_{t+1}) - V^{\pi_\theta^i}(s_t)
\end{equation}

where $r_t$ is the target policy reward.

Using advantage $\hat{A}^{\pi_\theta^i}(s_t, a_t)$ as an indication of the accuracy of $V^{\pi_\theta^i}(s_t)$, we define the reward \textbf{Advantage Weighted Target Value}:
\begin{equation}
    \hat{r}_t = ( 1 - \text{min}(\alpha\hat{A}^{\pi_\theta^i}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}^{\pi_\theta^i}(s_t)
    \label{eq:eq1}
\end{equation}

where the target policy value is weighted by the estimated advantage and $\alpha$ and $\beta$ are scaling factors tuned empirically (set to 0.15 and 0.01 respectively).

The target policy value function $V^{\pi_\theta^i}(s_t)$ has learned the value for states where the target policy has collected experience. Outside of these states, for example when the robot is activating a different policy, we expect the reward provided by the environment $r_t$, and the next state $s_{t+1}$ will not be consistent with what is expected by the target policy value function. Therefore, the advantage $\hat{A}^{\pi_\theta^i}(s_t, a_t)$ will not be close to zero, and $\hat{r}_t$ becomes small. Intuitively, for states where the target policy value function $V^{\pi_\theta^i}(s_t)$ is accurate, the target policy advantage $\hat{A}^{\pi_\theta^i}$ will be close to zero, thus the setup policy will learn to maximise $V^{\pi_\theta^i}$. State-action pairs where $\hat{A}^{\pi_\theta^i}(s_t, a_t)$ is far from zero will reduce the effect of an overconfident $V^{\pi_\theta^i}(s_t)$. 

\textbf{Extended Reward}: 
One issue with training setup policies is the delayed effect of actions, where once switched to the target policy, the setup policy is no longer acting on the environment or receiving a reward. Once the setup policy has transitioned to the target policy, we must provide the setup policy with information regarding the performance of the robot since switching. Our method for solving this problem is to provide the additional reward obtained \textit{after} switching, by including an extended reward in the rollout buffer of the setup policy. We add this extended reward to the last reward received running the setup policy: 
\begin{equation}
    % \text{Buffer}[\hat{r}][-1] \mathrel{+}= \hat{r}_t    
    \hat{r}_{final} = \hat{r}_{final\_prev} + \hat{r}_t 
\end{equation}
where $\hat{r}_{final\_prev}$ is the final reward entry received by the setup policy before switching, and $\hat{r_t}$ is the reward received at time $t$, after the setup policy has transitioned to the target policy. For algorithmic stability, we clear all but the last entry of the buffer after each training update. The last reward entry of the buffer becomes $\hat{r}_{final}$ for environment steps that continue after training. The procedure for training setup policies is provided in Algorithm~\ref{alg:setup}. Note that the termination variable $\tau_t$ (line 7) is either $\tau_\phi$ if the current policy is the setup policy, or $\tau_\theta$ if the current policy is the target policy.

\begin{algorithm}
	\caption{Setup Before Switching} 
	\begin{algorithmic}[1]
      \State Load Target Policy $\pi_\theta^i$. Load Default Policy $\pi_\theta^j$
      \State Initialise Setup Policy $\pi_\phi^i$ from the Default Policy
      \State Initialise Buffer
        \State Current Policy $\gets$ Default Policy
		\For {$iteration=1,2,\ldots$}
		    \While {not $done$}
    		    \State $a_t, \tau_t \sim $ Current Policy$(s_t)$ \Comment{$\tau$ is $\tau_\phi$ or $\tau_\theta$}
    		  %  (\tau is either \tau_\phi or \tau_\theta)
    		  %  \State ($\tau = \tau_\theta || \tau_\phi$)
    		    %\Comment{$\tau_\theta$ if Current Policy == }
    		    \State $s_{t+1}, r_t, done = env.step(a_t)$
    		    \If{Terrain detected}
    	            \State $\hat{A}^{\pi_\theta^i}(s_t, a_t) = r_t + \gamma V^{\pi_\theta^i}(s_{t+1}) - V^{\pi_\theta^i}(s_t)$
        		    \State $\hat{r}_t = (1 - \text{min}(\alpha\hat{A}^{\pi_\theta^i}(s_t, a_t)^2, 1))\cdot \beta V^{\pi_\theta^i}(s_t)$
        		    \If{Current Policy == Default Policy}
        		        \State Current Policy $\gets$ Setup Policy $\pi_\phi^i$
        		        \State $\tau_t \gets \tau_\phi$
            		\ElsIf{Current Policy == Setup Policy}
        		        \State Store $s_t$, $a_t$, $\hat{r}_t$, $\tau_\phi$ into Buffer
                        \If{Buffer Full}
                            \State PPO Training Update
                            \State Clear buffer (except last entry)
                        \EndIf
            		    \If {$\tau_\phi$}
            		        \State Current Policy $\gets$ Target Policy $\pi_\theta^i$
            		        \State $\tau_t \gets \tau_\theta$
            		    \EndIf
        			\ElsIf{$\tau_\theta$}
        			    \State Current Policy $\gets$ Default Policy $\pi_\theta^j$
        		    \EndIf
        		    \If{Current Policy != Setup Policy}
        			 %   \State Buffer$[\hat{r}][-1] \mathrel{+}= \hat{r}_t$
        			    \State $\hat{r}_{final} = \hat{r}_{final\_prev} + \hat{r}_t$ 
        			\EndIf
        		\EndIf
        		\State $s_t = s_{t+1}$
        	\EndWhile
		\EndFor
	\end{algorithmic} 
\label{alg:setup}
\end{algorithm}
% \vspace{15mm}
% \subsection{Terrain Classification}
% \label{sec:classifier}

% Classifier Network \textbf{TBD}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

We evaluate our method with a biped in simulation. Initial evaluations are performed with a single difficult terrain (Sec~\ref{sec:ablation}, Sec~\ref{sec:reward_choice}, Sec~\ref{sec:comparisons}), before adding more behaviours in Sec~\ref{sec:multi_terrain}. The difficult terrain is a sample of flat terrain with a single block 50 cm high, and 30 cm in length (in the forward direction of the robot), an example is shown in Fig.~\ref{fig:fig1}. We perform training and evaluation on a single terrain sample, starting the robot from a random $x$ (forward direction) uniformly sampled from (0.0, 2.2) $\si{\meter}$ before the terrain artifact, $y$ (strafe) uniformly sampled from (-0.6, 0.6) $\si{\meter}$, and $heading$ (yaw) uniformly sampled from (-0.3, 0.3) $\si{\radian}$. Setup policies are trained for a total of 10 million environment steps collected from 16 worker nodes, each performing a policy update every 2048 steps with averaged gradients. All experiments using a single terrain type are evaluated by pausing training and performing 100 evaluation runs, and recording both the Success percentage and Distance percentage. Success \% is defined as the average success rate to reach a goal location several meters past the terrain artifact. Distance \% is the average percentage of total terrain distance the agent successfully covered. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effect of Using Initialisation and Extended Reward}
\label{sec:ablation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We perform an ablation to study the effect of initialising the setup policy from the walking policy, and the effect of extending the reward after the setup policy has transitioned to the target policy. In all experiments the default policy is used until the terrain is detected, then the setup policy is activated until the termination signal $\tau_\phi$ indicates switching to the target policy, and $\tau_\theta$ then results in switching back to the default policy.

\begin{itemize}[leftmargin=*]

\item\textbf{Without Initialisation:} We evaluate our method without initialising the setup policy from the default walking policy, i.e. the setup policy is randomly initialised.

\item\textbf{Without Extended Reward:} We evaluate our method without including the reward after the setup policy has switched to the target policy. 

\item\textbf{Full Method:} Our method uses a setup policy initialised from the default walk policy, and receives reward signal after the setup policy has transitioned to the target policy. 

\end{itemize}

\begin{table}[h!]
    % \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Initialisation        & 38.8      & 73.2  \\
        Without Extended Reward       & 12.3      & 58.3  \\
        Full Method                          & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study for initialising setup policies from a default walk policy, and receiving an extended reward, for switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:results}
\end{table}

We can see that initialising the setup policy with the default walking policy and extending the reward improves learning outcomes as shown in Table~\ref{tab:results}, where our method achieves 82.2\% success compared to 38.8\% without initialisation from the default walking policy and 12.3\% without receiving the extended reward. 
% It is worth noting that training without initialisation from the walking policy required many more training steps to reach an asymptotic result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setup Policy Reward Choice}
\label{sec:reward_choice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For training the setup policy, we investigate several options for the reward provided at each timestep. For each reward type we evaluate with three different random seeds, results are shown in Fig~\ref{fig:results}.

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=\columnwidth]{images/results.png}
\hfill
\caption{We investigate several options for the reward function used to train a setup policy on the difficult jump terrain. We show the success rate (robot reaches several meters after the jump) during training for three different random seeds.}
\label{fig:results}
% \vspace{-3mm}
\end{figure}

\begin{itemize}[leftmargin=*]
\item\textbf{Original:} The reward afforded by the environment that is used to train the target policy: the reward encourages following an expert motion. 

\item\textbf{Constant:} At each timestep a constant reward of 1.5 is given.

\item\textbf{Target Torque:} We encourage the setup policy to match the output of the target policy by minimising the error: $\exp[-2.0\cdot (\pi_\phi(s_t) - \pi_\theta(s_t))^2]$. 

\item\textbf{Target Value:} We evaluate the effect of using the target policy value function as the reward for the setup policy. This is not the same as the original reward, as it is not provided by the environment, but by $\beta V^{\pi_\theta^i}(s_t)$, where $\beta$ is scaling factor 0.01.
%  maximising the target policy value function 

\item\textbf{Advantage Weighted Target Value:} We evaluate the reward introduced in Equation \ref{eq:eq1}.

\end{itemize}

It can be seen from Fig~\ref{fig:results} that a reward using \textbf{Advantage Weighted Target Value} performs better than other reward choices, achieving the highest average success rate (78.7\%). Using the target value reaches a success rate of 63.9\%. This disparity, and the large variation in the target value (green line), shows the effect of over estimation bias often seen with value functions, validating our idea that weighting the value by the advantage reduces the effect of this bias when training setup policies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparisons}
\label{sec:comparisons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We compare our method with several others, including end to end methods, without using setup policies, and a method that uses proximity prediction to train a transition policy~\cite{lee_composing_2019}.

\begin{table}[h!]
    % \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success\% & Distance\% \\
       \hline
        Single Policy                 & 0.0           & 11.3  \\
        Single Policy With Curriculum & 0.0           &  3.8 \\
        Without Setup Policies              & 1.5           & 51.3 \\
        Learn When to Switch          & 0.0           & 44.2  \\
        Proximity Prediction         & 51.3           & 82.4 \\
        Setup Policy (Ours)         & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success and average distance of the total length covered when switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:results_compare}
\end{table}

\begin{itemize}[leftmargin=*]

\begin{figure*}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth]{images/Fig1_2.png}
\includegraphics[width=\textwidth]{images/all.png}
\hfill
\caption{Setup policies enable a biped to transition between complex visuo-motor behaviours for traversing a sequence of diverse terrains.}
\label{fig:multi}
% \vspace{-3mm}
\end{figure*}

\item\textbf{Single Policy:} We train a single end to end policy on the terrain sample.

\item\textbf{Single Policy With Curriculum:} We utilise curriculum learning to train a single end to end policy on the terrain sample (using the method outlined in~\cite{tidd_guided_2020}).

\item\textbf{Without Setup Policies:} We switch to the target policy from the default policy as soon as the terrain oracle detects the next terrain.

\item\textbf{Learn When to Switch:} We collect data by switching from the default policy to the target policy at random distances from the Jump. We use supervised learning to learn when the robot is in a suitable state to switch. Details of this method is found in our previous work~\cite{tidd_learning_2021}.

\item\textbf{Proximity Prediction:} We follow the method defined by Lee et al.~\cite{lee_composing_2019} to train Transition Policies (one for each behaviour) using a proximity predictor function $P(s_t)$. $P(s_t)$ outputs a continuous value that indicates how close the agent is to a configuration that resulted in successful traversal. $P(s_t)$ is trained using supervised learning from success and failure buffers. The reward used to train the transition policy is the dense reward created by  $P(s_{t+1}) - P(s_{t})$, encouraging the agent to move closer to a configuration that results in successful switching. For accurate comparison we initialise the transition policy with weights from the walk policy, and utilise the terrain oracle for policy selection (the paper refers to a rule-based meta-policy in place of a terrain oracle~\cite{lee_composing_2019}).

\item\textbf{Setup Policy (Ours):} We follow Algorithm~\ref{alg:setup} to train setup policies. 

\end{itemize}

We can see from Table~\ref{tab:results_compare} that our method for developing setup policies performs the best (82.2\% success rate), compared to other methods. A single policy was unable to traverse the difficult jump terrain, even with an extended learning time and curriculum learning. The poor performance of \textbf{Single Policy With Curriculum} was the result of the robot not progressing through the curriculum, and as a consequence is unable to move without assistive forces during evaluation. In contrast, the single policy trains without assistive forces, so while the single policy still fails to complete the task, it is able to make forward progress when evaluated. These results highlight the difficulty of learning to walk and jump as a single behaviour. We show that setup policies are necessary for this problem, with \textbf{Without Setup Policies} unable to successfully traverse the terrain (1.5\% success). \textbf{Learning When to Switch} also performed poorly as there are very few states that overlap between the default policy and the target policy for the switch estimator to learn. The \textbf{Proximity Prediction} method was able to successfully traverse the jump 51.3\% of the time. It is worth noting that this method required approximately three times more training episodes than our method to reach the provided results, despite also being initialised from the default policy.

% The poor performance of \textbf{Single Policy With Curriculum} was the result of the robot not progressing through the curriculum, and as a consequence is unable to move without assistive forces.

These experiments show that for the difficult jump terrain, we require a specialised target policy dedicated to learning the complex jumping behaviour. We show that this specialised policy has a trajectory that does not overlap with the default policy, and thus setup policies are required. Our method for learning setup policies achieved the highest performance on this difficult task.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Multiple Terrain Types}
\label{sec:multi_terrain}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


For our final experiment we train setup policies for several additional terrain types. In total we now have modules for jumps, gaps, hurdles, stairs, and stepping stones. Fig~\ref{fig:multi} shows a sequence with each terrain type. We follow the pipeline shown in Fig~\ref{fig:fig2}a), where a terrain oracle determines which module should be selected. On selection, the setup policy is employed until the robot reaches a switch state ($\tau_\phi$), then switching to the target policy.
Termination criteria $\tau_\theta$ (introduced in Sec~\ref{sec:method}) determines when to switch back to the default policy for the jump obstacle only. All other policies resemble the behaviour of the default policy on flat terrain, i.e. we continue using the target policy after the terrain has been traversed for gaps, hurdles, stairs, and stepping stones, until the oracle determines the terrain has changed.

We evaluate with a sequence of each of the 5 terrain types, randomly shuffled before each run. We perform 1000 runs, with a total of 5000 various terrain types to be traversed. In Table~\ref{tab:multi_results} we show the average percentage of total distance travelled and success rate with and without using setup policies. A successful run in this scenario is defined as traversing the last terrain in the sequence. Table~\ref{tab:multi_breakdown} shows the failure count for each terrain type.
% Table~\ref{tab:multi_breakdown} shows the individual performance of the agent for each terrain type (number of successful traversals / total traversals).

\begin{table}[h!]
    % \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Setup Policies        & 1.9      & 36.3  \\
        % With setup policies       & \textbf{26.4}      & \textbf{53.2}  \\
        With Setup Policies       & \textbf{71.2}      & \textbf{80.2}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success rate and percentage of the total terrain length travelled from 1000 episodes of all 5 terrain types, randomly shuffled each episode.}
    \label{tab:multi_results}
\end{table}
\vspace{-2mm}

\begin{table}[h!]
    % \vspace{-9mm}
    \centering
    \begin{adjustbox}{min width=0.9\columnwidth}
    \begin{tabular}{cccccc}
                                      & Jump & Gap & Hurdle & Stairs & Steps \\
      \hline
        % Without setup policies       & 710      & 90  & \textbf{43} &  \textbf{20} & \textbf{90}  \\
        Without Setup Policies       & 782      & 52  & \textbf{36} &  \textbf{31} & \textbf{86}  \\
        % With setup policies        & \textbf{420}      & \textbf{70}  & 73 & 36 & 144 \\
        With Setup Policies        & \textbf{36}      & \textbf{48}  & 43 & 65 & 96 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Number of failures by terrain type from 1000 episodes of all 5 terrain types, randomly shuffled each episode.}
    \label{tab:multi_breakdown}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Setup Policies        & 68.2      & 78.1  \\
        With Setup Policies       & \textbf{76.7}      & \textbf{84.6}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success rate and percentage of the total terrain length travelled from 1000 episodes of 4 terrain types \textbf{(without the jump terrain)}, randomly shuffled each episode}
    \label{tab:multi_results_no_jumps}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{min width=0.82\columnwidth}
    \begin{tabular}{ccccc}
                                      & Gap & Hurdle & Stairs & Steps \\
      \hline
        Without Setup Policies       & 74  & \textbf{41} &  64 & 142  \\
        With Setup Policies        &  \textbf{44}  & 51 & \textbf{49} & \textbf{90} \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Number of failures by terrain type from 1000 episodes of 4 terrain types \textbf{(without the jump terrain)}, randomly shuffled each episode.}
    \label{tab:multi_breakdown_no_jumps}
\end{table}
\vspace{-2mm}
% \newpage
% \newline
% \vspace{-6mm}
We can see from Table~\ref{tab:multi_results} that setup policies improve the success rate compared to switching policies without the intermediate policy (71.2\% success compared to 1.9\%). Table~\ref{tab:multi_breakdown} provides a breakdown of the number of times the robot failed on each terrain. From Table~\ref{tab:multi_breakdown} we can see that setup policies are most critical for traversing the difficult jump terrain (reducing the failures from 782 to 36), though we also see improvements for gap terrain. 

\vspace{2.5mm}
To investigate further, we exclude the jump obstacle from the terrain sequence and still observe a significant benefit using setup policies. Table~\ref{tab:multi_results_no_jumps} shows the performance increase from 68.2\% to 76.7\% of successful traversals for 4 terrain types (excluding the jump obstacle). Common failure modes were seen when the robot veered from the walking line (centre y position) and was unable to recover in time for the next upcoming terrain. This often occurred before the stepping stone obstacle, which had the highest failure rate of the remaining terrain types (Table~\ref{tab:multi_breakdown_no_jumps}). Setup policies showed a clear benefit for each separate terrain type, however, we can see with the multi-terrain experiments there were cases where not using setup policies performed better (Table \ref{tab:multi_breakdown} and \ref{tab:multi_breakdown_no_jumps}). For the behaviours that did not require jumping with both feet switching early (\textbf{Without Setup Policies}) gave the robot time to correct its walking line before approaching the next terrain. 

% \vspace{2.5mm}
Despite the clear need for setup policies, we attribute failures to out of distribution states, i.e. the robot visits states in the terrain sequence that it does not experience when training on the individual terrain types. Earlier implementations found that training setup policies from less diverse starting locations resulted in poor performance when evaluated across multiple terrain types. In these experiments, setup policies successfully guided the robot during a set stage of the walking cycle, however were unable to control the robot when in other stages of walking, as were common after traversing different terrain types. Training setup policies for a wider range of states will be investigated in future work. 

% Furthermore, the performance of behaviours on each individual terrain type could be analysed to improve the generalisation of this method to new behaviours.

% investigation is required to improve the setup policies for this terrain (Table~\ref{tab:multi_breakdown_no_jumps}).


% While the results show that without setup policies the hurdle, stairs, and steps terrain appear to have less failures than running setup policies, we note that these terrains are visited far less times when running without setup policies due to significant failure with the jumps terrain.

% These results show the highest failure rate on the multi terrain setup is on the jump terrain, and that there is clear room for improvement on this terrain. 


%  For example, if the robot was on a gap, and using the gaps behaviour, then switches to the jumps setup policy to prepare for an upcoming jump, it will not necessarily be in a state that has been seen during training.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

It is common practice for legged robots to have separate locomotion policies to traverse different terrain conditions. We propose setup policies that enable smooth transition from the trajectory of one locomotion policy to the trajectory of a target policy for traversing difficult terrain with a dynamic biped. We use deep reinforcement learning to learn the setup policies for which we introduce a novel reward based on the Advantage Weighted Target Value, utilising the scaled value prediction of the target policy as the reward for the setup policy. 

In simulation experiments for transitioning from a walking policy to a jumping policy, we show using an in-between setup policy yields a higher success rate compared to using a single policy (0$\%$ success rate), or the two policies without the setup policy (from 1.5$\%$ success rate without setup policies to 82$\%$). We further show that our method is scalable to other terrain types, and demonstrate the effectiveness of the approach on a sequence of difficult terrain conditions, improving the success rate from 1.9$\%$ without setup policies to 71.2$\%$.

A limitation of our method is that setup policies are trained from a default walking policy. We would like to improve the scope of the setup policies such that a wider range of states are funnelled towards the target policy. The idea of utilising the advantage (estimated by the temporal difference (TD) error) as a confidence metric can be applied generally for region of attraction (RoA) expansion, safe reinforcement learning, and also for blending several behaviours for performing complex composite tasks. These ideas will be explored in future work. A significant assumption in this work is that we have access to a terrain oracle, removing this dependency will be required as we consider experiments in the real world.

% If we allowed further training of the target policies, our training method could be used to include more states and improve robustness. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% balance the last page
\addtolength{\textheight}{-2cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.
% might need that \newpage
% \ifCLASSOPTIONcaptionsoff
%   \newpage
% \fi


\bibliographystyle{IEEEtran}
\bibliography{references}
\end{document}



==> old/main_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
\label{sec:abstract}
Whats the main point I'm trying to make
\begin{itemize}
    \item In the real world we need multiple controllers, end-to-end is not an option, 
    \item distillation or progressive nets
    \item We want to leverage DRL to learn complex behaviours, but most 
\end{itemize}
\begin{itemize}
    \item 
\end{itemize}

Deep reinforcement learning (DRL) has been used for controlling legged platforms, removing some of the tuning of manual control methods. However, DRL policies behave as a black box, with little insight into where these policies work. Legged platforms require different policies to accomplish walking over specific terrain types, particularly for real world robots where developing policies may only be possible in constrained conditions. To combine several walking policies, we develop setup policies that prepare the robot for the upcoming terrain condition before switching to the required policy. We utilise advantage estimation as a local Lyapunov function as a reward signal for the setup policy. We show that we are awesome and can learn setup policies easily, and do wicked comparisons, and finally demonstrate our methods on lots of terrains, despite only training on single terrain conditions. We also learn when to switch. We verify our method in simulation with a biped and several terrain types.

\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:introduction}

Bipedal robots have the capability to cover a similar span of terrains as humans, therefore are an appealing locomotion option for robots in humancentric environments. However, designing a single locomotion controller that enables a platform to traverse every expected terrain is difficult. Also, legged platforms require treadmills, harnesses, and support mechanisms while controllers are developed, further restricting the operational scope of a single controller. A reasonable alternative to a monolithic control strategy is to design many dedicated controllers for specific terrain scenarios. Our work focuses on a modular approach to control design for a dynamic bipedal robot, that is required to traverse many complex terrain types.

Controlling a bipedal robot is a challenging control problem, particularly for difficult terrain conditions. In the real world, controllers for bipedal robots are designed with meticulous tuning, and a robot may require many controllers to perform complex maneuvers or traverse a range of terrain types. For dynamic platforms, switching from one controller to another must occur when the platform is in a state that common to both controllers. This means that the Region of Attraction (RoA), or the states that a controller can operate and converge to a stable goal state, must overlap from one controller to the next. Switching controllers when the platform is outside of the RoA of the receiving controller results in undesirable behaviour.


to sample of the expected work surface.

Big world, unreasonable to handle every situation.


Designing controllers for dynamic legged platforms is difficult. Typically.

Learning methods for developing policies remove some of the hand crating and tuning required to operate over challenging terrains, however learning methods  


Deep reinforcement learning (DRL) is an alternative to classical methods for developing controllers for legged platforms, though use on real platforms remains largely experimental. One of the challenges with DRL methods is knowing where policies work, that is, being confident in the stability of the current policy, as well as the secure transition to the next policy as the conditions require. 

For a biped to reliably walk over many domains, one approach is to design separate policies for each condition. Controller development for real platforms typically occurs in constrained conditions with a small sample of the terrain the robot is required to operate over. From previous work, curriculum learning can improve learning outcomes for policies trained on small samples of complex terrain types~\cite{ours1}~\cite{ours2}. For these complex policies to work together, we need to move the robot from the RoA of one policy to the RoA to the suitable policy for the upcoming terrain condition. 

We propose a method that uses a separate setup policy to move the robot to a safe region before switching. We utilise several policies that have been pre-trained on specific terrain conditions. For each terrain type, we learn a setup policy that guides the robot to the RoA of the respective terrain policy. 

Our contribution is a DRL policy to setup each pre-trained terrain policy, greatly improving the stability of switching between policies. We also use value estimation as a means of estimating the RoA of each policy, and thus when to switch. Our method is modular, and can be expanded to any number of terrain types. By combining black box policies, we are able to train specific policies, an system that can be applied to the real world. We train on a small sample of each terrain type, but can evaluate on a much larger set of terrain conditions.

The following work it set out like this:


Contributions: 
\begin{itemize}
    \item Introduce a modular approach to composing transitional between policies
    \item Leverage the policies value functions for reward
    
    \item Learn setup policies that prepare the robot for the next policy + learn where these work
    \item We learn when to use these policies 
    \item We show we are better than end to end, and bunch of comparisons
    \item we show we can combine several policies, without ever training on more than one terrain condition
    \item Same as last paper: Policies and setup policies only trained on a single terrain condition
    \item Closest paper is transition paper, but we use 18 DOF biped instead of 9 DOF walker. Much more complex terrain types, more complex perception (they use distance to artifact). They might train on the test set?
    \item Hopefully with new terrains the end-to-end won't work.
\end{itemize}
Limitations: 
\begin{itemize}
    \item Still need oracle terrain detector. (Don't think it's a problem to train a detector on all terrain types without using the policies i.e. from a human)
\end{itemize}
\textbf{Main graphic: setup policy into policy}

Problems/questions
\begin{itemize}
    \item Why not just train end to end?
    \item Does speaking about RoA make any sense? Am I using or learning anything about the RoA? - Can still show pca on state to see pol1 -> setup -> pol2
    \item this becomes very similar to transition policy paper
    
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:related_work}

Utilising multiple control primitives is common for dynamic platforms, whether controlled with classical~\cite{schaal_dynamic_2006}, or DRL approaches~\cite{lee_composing_2019}. By combining individual controllers the agent is able to be controlled through a larger span of states than any individual primitive. Developing primitives separately allows control design to be performed in a controlled setting, resulting in improved performance of individual behaviours~\cite{lee_robust_2019}.

In the classical control community, identifying where in the state controllers work allows the safe combination of primitives. Burridge et al introduce Sequential Composition, the idea that controllers can be chained through the overlap in their Region of Attraction (RoA)~\cite{burridge_sequential_1999}. Specifically, one controller moves the agent to the RoA of the next. The Region of Attraction for a controller is a subset of the state space that the agent will remain within while executing the respective controller, eventually converging to a goal set~\cite{berkenkamp_safe_2017}. A controller that is operated outside of its RoA is unstable. The challenge when combining control primitives is identifying this set of states for each controller, only switching when the agent is in a state suitable for the upcoming controller. For high dimensional dynamic robots it is difficult to determine the complete set of states in the RoA for a controller. All the primitive papers from the last paper.

\subsection{Hierarchical RL}


\subsection{Modular RL}
Wenlong Huang train Shared Modular Policies, a single policy is trained, for each actuator where the parameters are shared accross all limbs of all agents. Messages are passed between joints, enabling characters of different morphologies to learn forward motion using the same policy. Continuous control, 2D actors.



Learning based methods have demonstrated promise for legged platforms in recent years~\cite{}. 
in DRL

Safe learning by understanding where policies are stable is currently limited to low dimensional agents such as the inverted pendulum~\cite{najafi_learning_2016},~\cite{berkenkamp_safe_2017}. Berkenkamp et al identify the value function used by actor critic DRL methods exhibits similar properties to a Lyapunov function~\cite{berkenkamp_safe_2017}. Understanding where policies work for high dimensional agents remains challenging.

Our method trains setup policies similar to~\cite{lee_composing_2019} with a more complex 3D agent with many difficult terrain types. We hypothesis that the advantage estimate provides a better estimate of the Lyapunov function than the value function, providing a dense reward for our setup policies,



Classical methods follow 


This is a subset of the state space that is forward invariant so that any state trajectory that starts within this set stays within it for all times and converges to a goal state eventually.~\cite{berkenkamp_safe_2017}
\begin{itemize}
    \item Classical methods for bipeds with primitives
    \item DRL methods for biped with primitives
    \item More on lyapanouv stability
\end{itemize}
\textbf{Look at references for transition paper}
\begin{itemize}
    \item MARL - Multi Agent RL Ryan Lowe, Yi Wu, Aviv Tamar, Jean Harb, OpenAI Pieter Abbeel, and Igor Mordatch. Multi-agent
actor-critic for mixed cooperative-competitive environments. In Advances in Neural Information
Processing Systems, pp. 6379–6390, 2017. 
    \item skill behavior diversification (SBD)~\cite{youngwoon lee}
    \item  adding Qfunctions (Haarnoja et al., 2018a), additive composition (Qureshi et al., 2020; Goyal et al., 2020), or
multiplicative composition (Peng et al., 2019). 
    \item n. For cooperative tasks, communication mechanisms (Sukhbaatar et al., 2016; Peng et al.,
2017; Jiang \& Lu, 2018), sharing policy parameters (Gupta et al., 2017), and decentralized actor
with centralized critic (Lowe et al., 2017; Foerster et al., 2018) have been actively used. However,
these approaches suffer from the credit assignment problem (Sutton, 1984) among agents and the
lazy agent problem (Sunehag et al., 2018).
\item Pattie Maes and Rodney A Brooks. Learning to coordinate behaviors. In Association for the
Advancement of Artificial Intelligence, volume 90, pp. 796–802, 1990
\end{itemize}

Comparisons: 
\begin{itemize}
    \item Transition paper, why are we better?
    \item Previous heuristic methods?
    \item Previous learn when to switch method
    \item end-to-end, DQN 
\end{itemize}
% \section{Background}

% \input{sections/background.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\label{sec:method}
% \begin{figure*}[tb!]
% % \vspace{2mm}
% \centering
% \includegraphics[width=1.2\columnwidth]{images/Fig2.png}
% \caption{.}
% \label{fig:2}
% \vspace{-3mm}
% \end{figure*}

\subsection{Problem Description}
\label{sec:problem}

We experiment with a dynamic biped (12 torque controlled joints) in simulation (Pybullet~\cite{coumans_pybullet_nodate}). Given a set of terrain conditions, and a pre-trained policy for each terrain type, we wish to autonomously traverse any combination of terrains within the set. The set of terrains is variable, meaning we can add a new terrain to the set (with its associated policy). A final condition we impose is that we only have access to a single terrain type during training. This is to mimic real world conditions where setting up an exhaustive set of terrain examples during controller development is impractical.

We propose a modular reinforcement learning approach to solving this problem, where each terrain type will have a separate module. We identify three primary components required for each module.
\begin{itemize}
    \item Policy and Value function (provided)
    \item Setup Policy
    \item Selection Policy
\end{itemize}

Policies are trained using a curriculum learning introduced in~\cite{my_work}.

% \subsection{Region of Attraction Hierarchy}
% \label{sec:roa_method}

% Dynamic robots that require switching from one controller to another must have an overlap in admissible states. Admissible states refer to the region of attraction

% We identify a region of attraction hierarchy for policies controlling dynamic locomotion platforms. In the high level, policies must reach a region before the terrain (distance and heading to the terrain). In the low level the robot must be in a configuration, traditional region of attraction, (CoM position and velocity, joint configuration) - I wonder if this should be a separate thing, like just the explanation, and in the results we can show the effect of moving the 2D body around an artifact, and PCA on the initial joint configurations from a known 2D location? Graphics for both?

% \begin{itemize}
%     \item Given a set of policies trained on a single terrain
%     \item For each policy collect image data, train classifier
%     \item Train DQN and Setup policy -> DQN with advantage estimates, Setup policy with our reward function
%     \item Test our system on any number of terrains. i.e. 
%         \begin{itemize}
%             \item Detect terrain
%             \item Run setup policy. When DQN, switch
%             \item Run policy, When DQN, end
%         \end{itemize}
    
    
% \end{itemize}

% \subsection{Setup Policy}
% \label{sec:setup_method}

% We the robot is close to the high level region of attraction of the target policy, we need the robot to prepare for the target policy. For example, following a walking policy the robot is now in front of a large ledge that requires a jump with both feet together. We cannot simply switch to the jump policy from the walking policy, (NEED TO SHOW THIS). Instead we develop an intermediate setup policy that moves the robot from the walking policy into the region of attraction of the jump policy.

% The setup policy is trained with reinforcement learning to optimise a novel reward. We first introduce the advantage of

% We estimate the region of attraction of the target policy 

% Oracle terrain detector -> setup policy -> policy

% The setup policy is trained for a fixed length.

% Draw parallels from control theory where we look for a Lyapunov function 
% We use a RoA estimation as a reward signal for the setup policy. 



\begin{equation}
    \mathbb{E}_{x\in A}
    \mathop{\mathbb{E}}
\end{equation}
% \begin{equation}
%     \hat{V}(s_t) = \sum_{t=0}^T \gamma^t \hat{r_t}
% \end{equation}

% \begin{equation}
%     \hat{V}(s_t) = \sum_{t=0}^T \gamma^{t-1} \hat{r_t}
% \end{equation}

\begin{equation}
    \hat{V}(s_t) = \mathbb{E}_{t}^T \gamma^{t-1} \hat{r_t}
\end{equation}

\begin{equation}
    A_{target}(s_t, a_t) = r_{target} + V_{target}(s_{t+1}) - V_{target}(s_t)
\end{equation}

\begin{equation}
    r_t = ( 1 - \text{min}(A_{target}(s_t, a_t)^2,1) ) \cdot V_{target}(s_t)
\end{equation}

\begin{equation}
    r_t = (1 - A_{target}) \cdot V_{target}
\end{equation}

\subsection{Selection Policy}
\label{sec:selection_method}

Detect terrain (classifier or oracle)
- Run setup policy
- On Selection policy: switch to policy
- Run Policy
- On Selection policy: switch to default policy

% \begin{algorithm}
%     \caption{Euclid’s algorithm}
%     \label{euclid}
%     \begin{algorithmic}[1]
%         \State Load Policy
%         \State Initialise Setup Policy from Default Policy
%         \State $r\gets a \bmod b$
%         \While{$r\not=0$} \Comment{We have the answer if r is 0}
%             \State $a \gets b$
%             \State $b \gets r$
%             \State $r \gets a \bmod b$
%         \EndWhile\label{euclidendwhile}
%         \State \textbf{return} $b$\Comment{The gcd is b}
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
%     \caption{Euclid’s algorithm}
%     \label{euclid}
%     \begin{algorithmic}[1] % The number tells where the line numbering should start
%         \Procedure{Euclid}{$a,b$} \Comment{The g.c.d. of a and b}
%             \State $r\gets a \bmod b$
%             \While{$r\not=0$} \Comment{We have the answer if r is 0}
%                 \State $a \gets b$
%                 \State $b \gets r$
%                 \State $r \gets a \bmod b$
%             \EndWhile\label{euclidendwhile}
%             \State \textbf{return} $b$\Comment{The gcd is b}
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \SetAlgoLined
% \KwResult{Write here the result }
%  initialization\;
%  \While{While condition}{
%   instructions\;
%   \eIf{condition}{
%   instructions1\;
%   instructions2\;
%   }{
%   instructions3\;
%   }
%  }
%  \caption{How to write algorithms}
% \end{algorithm}

% \begin{algorithm}
% 	\caption{PPO} 
% 	\begin{algorithmic}[1]
% 	    \State Load Terrain Policy
% 	    \State Load Default Policy
% 	    \State Set Module to default
% 	    \State Initialise weights for Setup Policy and Selection Policy 
% 		\For {$iteration=1,2,\ldots$}
% 		    \If {Terrain detection}
% 		        \State Set Module to Terrain
% 		        \For {$iteration=1,2,\ldots$}
%     		        \State Run Setup Policy for Terrain
%     		        \if Selection Policy Terrain
%     		        \Stage Run Policy for Terrain
%     		        \if On Selection Policy Default
%     		        \State Run Default Policy
%     		    \EndFor
% 			\For {$actor=1,2,\ldots,N$}
% 				\State Run policy $\pi_{\theta_{old}}$ in environment for $T$ time steps
% 				\State Compute advantage estimates $\hat{A}_{1},\ldots,\hat{A}_{T}$
% 			\EndFor
% 			\State Optimize surrogate $L$ wrt. $\theta$, with $K$ epochs and minibatch size $M\leq NT$
% 			\State $\theta_{old}\leftarrow\theta$
% 		\EndFor
% 	\end{algorithmic} 
% \end{algorithm}


\begin{algorithm}
	\caption{Setup Before Switching} 
	\begin{algorithmic}[1]
      \State Load Terrain Policy
      \State Initialise Setup Policy from Default Policy
      \State Initialise Selection Policy
      \State Initialise Buffer, $\epsilon = 1.0$
		\For {$iteration=1,2,\ldots$}
		    \If{Terrain detected}
		        \If{$\epsilon < random()$}
    		        \State Current Policy $\gets$ $\argmax$ Selection Policy \Comment{Setup Policy or Terrain Policy}
    		    \Else
    		        \State Current Policy $\gets$ Oracle
    		    \EndIf
		        \State $r_t = (1 - A_{tp}(s_t, a_t)^2)\cdot V_{tp}(s_t)$
		        \If{Current Policy == Setup Policy}
                    \State Store $s_t$, $a_t$, $r_t$ into Buffer
                    \If{Buffer Full}
                        \State PPO Training Update
                        \State Clear buffer
                    \EndIf
    			\Else
    			    \State Setup Policy Last $r \mathrel{+}= r_t$
    			\EndIf
    		\Else
    		    \State Current Policy $\gets$ Default Policy
    		\EndIf
		    \State Run Current Policy
    		\State $\epsilon = 1-2\cdot\text{Success}$
		\EndFor
	\end{algorithmic} 
\end{algorithm}

% \begin{algorithm}
% 	\caption{PPO} 
% 	\begin{algorithmic}[1]
% 		\For {$iteration=1,2,\ldots$}
% 			\For {$actor=1,2,\ldots,N$}
% 				\State Run policy $\pi_{\theta_{old}}$ in environment for $T$ time steps
% 				\State Compute advantage estimates $\hat{A}_{1},\ldots,\hat{A}_{T}$
% 			\EndFor
% 			\State Optimize surrogate $L$ wrt. $\theta$, with $K$ epochs and minibatch size $M\leq NT$
% 			\State $\theta_{old}\leftarrow\theta$
% 		\EndFor
% 	\end{algorithmic} 
% \end{algorithm}

\begin{itemize}
    \item Sample n trajectories from goal set (unperturbed, achieve success criteria)
    \item \textbf{Pick a few good candidates: from the goal trajectories, add a bit of noise and run, see which ones succeed the most, and track those trajectories, or setup to single good robot poses}
    \item setup policy = target policy
    \item On detection: find closest trajectory from sampled = target trajectory
    \item Track target trajectory (same reward as policies), with perturbations, starting from random policy, in random pose. Train with fixed number of timesteps (one step = 60 steps).
    \item Need way to know when to switch (distance to target trajectory?), or switch after fixed number of timesteps
\end{itemize}
\textbf{Figure 2: Similar flow to last paper: detect terrain $j \rightarrow$ setup policy $j \rightarrow$ ready to switch $ \rightarrow$ switch to j}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

\subsection{Setup Policies}
\label{sec:setup_results}
Comparisons

\subsection{Policy Selection}
\label{sec:selection_results}

\subsection{Various Terrains}
\label{sec:terrains}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> old_diff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
\label{sec:abstract}
Dynamic platforms that operate over many unique terrain conditions typically require \DIFdelbegin \DIFdel{multiple controllers}\DIFdelend \DIFaddbegin \DIFadd{many behaviours}\DIFaddend . To transition safely\DIFdelbegin \DIFdel{between controllers}\DIFdelend , there must be an overlap of states between adjacent controllers. We develop a novel method for training \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend that bridge the trajectories between pre-trained Deep Reinforcement Learning (DRL) policies. We demonstrate our method with a simulated biped traversing a difficult jump terrain, where a single policy fails to learn the task, and switching between pre-trained policies without \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend also fails. We perform an ablation of key components of our system, and show that our method outperforms others that learn transition policies. We demonstrate our method with several difficult and diverse terrain types, and show that we can use \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend as part of a modular control suite to successfully traverse a sequence of complex terrains. We show that using \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend improves the success rate for traversing a single difficult jump terrain (from 1.5$\%$ success rate without \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend to 82$\%$), and \DIFdelbegin \DIFdel{a sequence of various terrains (from 6.8}\DIFdelend \DIFaddbegin \DIFadd{traversing a random sequence of difficult obstacles (from 1.9}\DIFaddend $\%$ without \DIFdelbegin \DIFdel{Setup Policies to 26.4}\DIFdelend \DIFaddbegin \DIFadd{setup policies to 71.2}\DIFaddend $\%$).


% \textbf{why do I care?}
% , as it may not be possible to safely switch between controllers outside of the overlapping states.
\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:introduction}

Bipedal robots have the capability to cover a span of terrains that humans can traverse. This makes bipeds an appealing locomotion option for robots in human environments. It is impractical, however, to design a single controller that works over all required environments, particularly if all conditions are not known a priori. For robots to be able to perform a number of diverse behaviours, it is desirable for a control suite to be modular, where any number of behaviours can be added with minimal retraining.

% included in the control repertoire. 
% Ideally, as new conditions are identified and new controllers become available, the new behaviours can be added to the control suite with minimal retraining.

Deep Reinforcement Learning (DRL) is an appealing method for developing \DIFaddbegin \DIFadd{visuo-motor }\DIFaddend behaviours for legged platforms. However, such DRL policies are usually trained \DIFdelbegin \DIFdel{in the same }\DIFdelend \DIFaddbegin \DIFadd{on the }\DIFaddend terrain they are expected to operate, though it is unlikely that the agent would have access to a complete set of terrain conditions during policy training before deployment. Controllers for dynamic platforms are typically developed and tuned with \DIFdelbegin \DIFdel{harnesses and treadmills }\DIFdelend \DIFaddbegin \DIFadd{safety harnesses and human supervisors }\DIFaddend in order to minimise potential damage to the robot and the environment. These restrictions limit the development of controllers over an exhaustive collection of terrain conditions. Furthermore, \DIFdelbegin \DIFdel{it is preferable to not re-design }\DIFdelend \DIFaddbegin \DIFadd{modifying }\DIFaddend controllers that have already been tuned \DIFdelbegin \DIFdel{, whereas }\DIFdelend \DIFaddbegin \DIFadd{is costly, for example }\DIFaddend DRL methods typically require retraining if \DIFdelbegin \DIFdel{the target conditions are evolved to included new terrains }\DIFdelend \DIFaddbegin \DIFadd{new terrains are introduced}\DIFaddend . We propose training a \textit{\DIFdelbegin \DIFdel{Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policy}\DIFaddend } to transition between two pre-trained policies targeting different terrains.

A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over if controllers are switched when the robot is not in a safe region for the subsequent controller. Figure~\ref{fig:fig1} shows our primary contribution: a \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend that prepares the robot for the necessary controller to traverse the upcoming terrain obstacle. With our method, we can transition between existing behaviours, allowing pre-trained DRL policies to be combined. 

% We propose a modular approach to developing a control suite for a biped expected to traverse a number of difficult terrain artifacts, where all terrain conditions are not known when training each module. A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over. Figure~\ref{fig:fig1} shows our primary contribution: a setup policy that prepares the robot for the upcoming terrain artifact. With our method, we can safely transition between behaviours that are developed separately, such that any number of pre-trained DRL policies can be combined, without any re-training of low level policies.  

\begin{figure}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth,natwidth=610,natheight=642]{images/Fig1.png}
\includegraphics[width=\columnwidth]{images/Fig1.png}
% \includegraphics[width=\columnwidth]{images/Fig1_err.png}
\hfill
\caption{As the robot approaches a difficult terrain artifact, it must move into position for target policy \DIFdelbeginFL \DIFdelFL{$j$}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{$i$}\DIFaddendFL . The trajectory of the walking policy \DIFdelbeginFL \DIFdelFL{$i$ }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{$j$ }\DIFaddendFL (shown with a blue line), does not intersect with the trajectory of the target policy \DIFdelbeginFL \DIFdelFL{$j$ }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{$i$ }\DIFaddendFL (green line). Our setup policy provides a trajectory that prepares the robot for the upcoming target policy (orange line).}
\label{fig:fig1}
% \vspace{-3mm}
\end{figure}
% How can we leverage subpolicy learning to improve learning outcomes?
Our contributions are as follows:
\begin{itemize}
    \item Using pre-trained policies, we develop \DIFdelbegin \DIFdel{a }\DIFdelend \textbf{\DIFdelbegin \DIFdel{Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policies}\DIFaddend } that significantly \DIFdelbegin \DIFdel{improves }\DIFdelend \DIFaddbegin \DIFadd{improve }\DIFaddend the success rate from transitioning from a default walking policy to a target policy (from 1.5$\%$ success rate without \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend to 82$\%$ for a difficult \DIFdelbegin \DIFdel{0.7}\DIFdelend \DIFaddbegin \DIFadd{0.5}\DIFaddend m jump). The setup policy also learns when to switch to the target policy. 
    \item We introduce a novel reward, called \textbf{Advantage Weighted Target Value}, \DIFdelbegin \DIFdel{based on the performance of the subsequent }\DIFdelend \DIFaddbegin \DIFadd{guiding the robot towards the target }\DIFaddend policy.
    \item We show that we can use \DIFdelbegin \DIFdel{our }\DIFdelend setup policies with several difficult terrain types, allowing for a modular control suite, combining \DIFdelbegin \DIFdel{policies }\DIFdelend \DIFaddbegin \DIFadd{behaviours }\DIFaddend that have been trained separately \DIFaddbegin \DIFadd{without any retraining of low level policies}\DIFaddend .
\end{itemize}

% The organization of this paper is as follows. After reviewing the relevant literature in Sec~\ref{sec:related_work}, we define the problem in Sec~\ref{sec:problem}, the learning algorithm in Sec~\ref{sec:ppo}, and our method for developing setup policies in Sec~\ref{sec:setup}. Our experimental results and comparisons are shown in Sec~\ref{sec:experiments}. Finally, we conclude with a brief discussion in Sec~\ref{sec:conclusion}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:related_work}
% Related work should also be story, starting from the start of the problem, highlighting what is missing, and refining to the specific paper that is closest to ours. Goal is to find gaps, start broad, and funnel into specifics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Deep reinforcement learning (DRL) has demonstrated impressive results for locomotion tasks in recent works~\DIFdelbegin \DIFdel{\mbox{%DIFAUXCMD
\cite{schulman_proximal_2017, heess_emergence_2017, peng_deeploco_2017, peng_deepmimic_2018, xie_allsteps_2020}}\hspace{0pt}%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{heess_emergence_2017, peng_deeploco_2017, peng_deepmimic_2018, xie_allsteps_2020}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend . Typically DRL policies optimise a single reward function, as new environments and behaviours are introduced costly retraining is required. \DIFaddbegin \DIFadd{Single policies have demonstrated locomotion over various terrains for simple 2D cases \mbox{%DIFAUXCMD
\cite{song_recurrent_2018}}\hspace{0pt}%DIFAUXCMD
, and impressive quadruped behaviours \mbox{%DIFAUXCMD
\cite{lee_learning_2020, rudin_learning_2021}}\hspace{0pt}%DIFAUXCMD
, however, for many scenarios multiple policies are often required. }\DIFaddend Furthermore, developing a single policy to perform multiple behaviours can degrade the performance of each behaviour~\cite{lee_robust_2019}.

Hierarchical reinforcement learning (HRL) offers flexibility through architecture, \DIFdelbegin \DIFdel{involving }\DIFdelend \DIFaddbegin \DIFadd{by }\DIFaddend training all segments of the hierarchy concurrently~\cite{sutton_between_1999, bacon_option-critic_2018, frans_meta_2018,peng_deeploco_2017}, or training parts of the hierarchy separately~\cite{merel_hierarchical_2019},~\cite{lee_composing_2019}.  When trained together, HRL can improve task level outcomes, such as steering and object tracking~\cite{peng_deeploco_2017}, or improve learning efficiency by reusing low level skills across multiple high level tasks~\cite{frans_meta_2018}. When trained separately, low level controllers can be refined efficiently using prior knowledge, such as by utilising motion capture data~\cite{peng_deepmimic_2018, merel_hierarchical_2019, peng_mcp_2019} or behavioural cloning~\cite{strudel_learning_2020}. For robotics applications it may be difficult to develop controllers for multiple behaviours simultaneously. Using pre-trained primitives can break up a large difficult problem into smaller solvable sub-problems~\cite{schaal_dynamic_2006}.

Using pre-trained policies requires \DIFdelbegin \DIFdel{a }\DIFdelend suitable handling of transitions between behaviours. Faloutsos et al\DIFaddbegin \DIFadd{.}\DIFaddend ~\cite{faloutsos_composable_2001} learns pre and post-conditions for each controller, such that switching only occurs when these conditions have been satisfied. DeepMimic by Peng et al\DIFaddbegin \DIFadd{.}\DIFaddend ~\cite{peng_deepmimic_2018} combines pre-trained behaviours learned from motion capture, with reliance on a phase variable to determine when one behaviour has been completed. Policy sketches introduce a hierarchical method that uses task specific policies, with each task performed in sequence~\cite{andreas_modular_2017}. CompILE uses soft boundaries between task segments~\cite{kipf_compile_2019}. Work by Peng et al\DIFaddbegin \DIFadd{.}\DIFaddend ~\cite{peng_terrain-adaptive_2016} trains several actor-critic control policies, modulated by the highest critic value in \DIFdelbegin \DIFdel{an }\DIFdelend \DIFaddbegin \DIFadd{a }\DIFaddend given state. For these examples there must be a reasonable state overlap between \DIFdelbegin \DIFdel{sequential }\DIFdelend controllers.

Other methods that combine pre-trained behaviours learn latent representations of skills~\cite{pertsch_accelerating_2020} or primitives~\cite{ha_distilling_2020}, enabling interpolation in the latent space. From an offline dataset of experience, Pertsch et al\DIFdelbegin \DIFdel{~\mbox{%DIFAUXCMD
\cite{pertsch_accelerating_2020} }\hspace{0pt}%DIFAUXCMD
are }\DIFdelend \DIFaddbegin \DIFadd{.~\mbox{%DIFAUXCMD
\cite{pertsch_accelerating_2020} }\hspace{0pt}%DIFAUXCMD
were }\DIFaddend able to combine low level controllers in manipulation tasks and locomotion \DIFdelbegin \DIFdel{task }\DIFdelend for a multi-legged agent. Ha et al\DIFaddbegin \DIFadd{.}\DIFaddend ~\cite{ha_distilling_2020} utilise motion capture to learn latent representations of primitives, then use model predictive control \DIFdelbegin \DIFdel{for the high level navigation of }\DIFdelend \DIFaddbegin \DIFadd{to navigate with }\DIFaddend a high dimensional humanoid. The FeUdal approach learns a master policy that modulates
low-level policies using a learned goal signal~\cite{vezhnevets_feudal_2017}. Work by Peng et al\DIFaddbegin \DIFadd{.}\DIFaddend ~\cite{peng_mcp_2019} combines pre-trained policies using a gating function that learns a multiplicative combination of actions. In our previous work~\cite{tidd_learning_2021}, we learn when to switch between low level primitives for a simulated biped using data collected by randomly switching between behaviours. Interpolation between behaviours yields natural transitions~\cite{xu_hierarchical_2020}\DIFdelbegin \DIFdel{, however in }\DIFdelend \DIFaddbegin \DIFadd{. Yang et al.~\mbox{%DIFAUXCMD
\cite{yang_multi_2020} }\hspace{0pt}%DIFAUXCMD
learn a gating neural network to blend several separate expert neural network policies to perform trotting, steering, and fall recovery in real-world experiments with a quadruped. Da et al.~\mbox{%DIFAUXCMD
\cite{da_supervised_2017} }\hspace{0pt}%DIFAUXCMD
use supervised learning to train a control policy for a biped from several manually derived controllers to perform periodic and transitional gaits on flat and sloped ground. In }\DIFaddend each of these approaches, experience from all behaviours must be available during training. 

For dynamic platforms, where separate controllers occupy different subsets of the state, changing behaviours may \DIFdelbegin \DIFdel{not result in stable behaviour }\DIFdelend \DIFaddbegin \DIFadd{result in instability }\DIFaddend if there is no overlap between controllers. Lee et al\DIFaddbegin \DIFadd{.}\DIFaddend ~\cite{lee_composing_2019} learn a proximity predictor to train a transition policy to \DIFdelbegin \DIFdel{get }\DIFdelend \DIFaddbegin \DIFadd{guide }\DIFaddend an agent to the initial state required by the next controller. Locomotion experiments are demonstrated with a 2D planar walker, where learning occurs by training with all terrain conditions. \DIFdelbegin \DIFdel{Our setup policies also use an intermediate controller, however we }\DIFdelend \DIFaddbegin \DIFadd{We }\DIFaddend show that our method performs more reliably (with a higher success rate)\DIFdelbegin \DIFdel{while performing complex behaviours with a 3D biped, despite only }\DIFdelend \DIFaddbegin \DIFadd{, despite }\DIFaddend training with experience from a single terrain \DIFdelbegin \DIFdel{obstacle for each behaviour}\DIFdelend \DIFaddbegin \DIFadd{type. Our setup policies learn to transition between complex behaviours with a 3D biped in a simulation environment using a depth image to perceive the terrain}\DIFaddend . 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Berkencamp, and mace use values to estimate when to use controllers.
% Composing paper. Something more specific about our method: advantage weighted value, this is a primary contribution. Training on sample only. Scaling to any number of policies, only needing data to train classifier, (no training of policies on anything but samples).


% sequential decision making tasks
% with greater sample efficiency than their non-hierarchical counterparts because hierarchical agents can break down tasks into sets of subtasks that only require short
% sequences of decisions.LEARNING MULTI-LEVEL HIERARCHIES WITH
% HINDSIGHT Andrew Levy , Hierarchical Actor-Critic (HAC), . Yet, learning multiple
% levels of policies in parallel is hard because it is inherently unstable: changes in
% a policy at one level of the hierarchy may cause changes in the transition and reward functions at higher levels in the hierarchy, making it difficult to jointly learn
% multiple levels of policies.  The main idea behind HAC is to train each level of the
% hierarchy independently of the lower levels by training each level as if the lower
% level policies are already optimal.

% HIRO Data-Efficient Hierarchical Reinforcement Learning Ofir Nachum - Use reward relabeling - High level give goals to low level. rewards from the environment are reused, temporal abstraction, off-policy.


% The first category lets a high-level policy select a low-level skill to execute [13, 14, 15, 28],
% which we refer to as the selector methods. In the second category, a subgoal is set for the low level by
% high-level policies [8, 9, 11, 10, 25], which we refer to as subgoal-based methods.

% % \subsection{Hierarchical RL}

% % \subsection{Transition Policies and Modular RL}
% % \textbf{ TODO Transition papers
% \begin{itemize}
%     \item sutton \cite{Sutton2017ReinforcementA.G.}
%     \item HRL \cite{sutton_between_1999} - introduces options, a framework for splitting mdp into temporally abstracted options.
%     \item m, HRL with Advantage function-based Auxiliary Rewards \cite{li et al} - Use the advantage of the high level policy as dense reward signal for an otherwise sparse reward problem,  improving pre-trained low level policies for navigation with legged locomotion.
%     \item 
%     \item COMPOSING COMPLEX SKILLS BY LEARNING TRANSITION POLICIES~\cite{lee_composing_2019}
%     \item MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies~\cite{peng_mcp_2019}
%     \item  MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies

%     \item Robust Recovery Controller for a Quadrupedal Robot using Deep Reinforcement Learning\cite{lee_robust_2019}
%     \item Modular multitask reinforcement learning with
% policy sketches \cite{andreas_modular_2017}
%     \item The option-critic architecture \cite{bacon_option-critic_2018}
%     \item DIVIDE-AND-CONQUER REINFORCEMENT LEARNING \cite{ghosh_divide-and-conquer_2018}
%     \item distillation - PLAID
%     \item progressive learning? progressive nets?
%     \item FeUdal Networks for Hierarchical Reinforcement Learning Alexander Sasha Vezhnevets \cite{vezhnevets_feudal_2017}
%     \item Terrain-Adaptive Locomotion Skills Using Deep Reinforcement Learning peng: relies on taking an action based on its value, (overestimated)
%     \item bekencamp - value to predict roa of pendulum (overestimated)
% \end{itemize}


% \begin{itemize}
%     \item Composable Controllers for Physics-Based Character Animation~\cite{faloutsos_composable_2001}
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\label{sec:method}

In this section we describe the problem we are solving and our method for training setup policies. 

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=\columnwidth]{images/Fig2.png}}
\hfill
\subfloat[]{\includegraphics[width=\columnwidth]{images/Fig3.png}}
% \hfill
\caption{a) shows the modular pipeline. A terrain classifier selects which module should be utilised, and the torque from the output of the selected module is applied to the robot, returning robot state and depth image. b) Each module is pre-trained on a single terrain type. The \DIFdelbeginFL \DIFdelFL{Target Policy }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{target policy }\DIFaddendFL has been designed to traverse a specific terrain condition. The \DIFdelbeginFL \DIFdelFL{Setup Policy }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{setup policy }\DIFaddendFL guides the trajectory of the robot from a default walking controller to the \DIFdelbeginFL \DIFdelFL{Target Policy}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{target policy}\DIFaddendFL , also learning when to switch to the \DIFdelbeginFL \DIFdelFL{Target Policy}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{target policy}\DIFaddendFL .}
\label{fig:fig2}
% \vspace{-3mm}
\end{figure}

\subsection{Problem Description}
\label{sec:problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We investigate composing controllers for a dynamic platform with \DIFdelbegin \DIFdel{little }\DIFdelend \DIFaddbegin \DIFadd{narrow }\DIFaddend or no state overlap between adjacent behaviours. An example of where this occurs when a bipedal robot performs a jump over a large block. In this scenario, the robot walks up to the block using a walking policy and then performs a jump with a terrain-specific \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend , where the behaviour involves jumping with both feet. Fig~\ref{fig:fig1} shows that the trajectory of the walk policy does not intersect with the trajectory of the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend , therefore we require an intermediate policy. While it may be possible to improve the robustness of the target policies after they have been trained (i.e. to include states visited by the walk policy), we consider the case where target behaviours and value functions are provided as a black box and are therefore immutable. Our agent has 12 torque controlled actuators, simulated in \DIFdelbegin \DIFdel{Pybullet}\DIFdelend \DIFaddbegin \DIFadd{PyBullet}\DIFaddend ~\cite{coumans_pybullet_2020}.

We select which terrain module to employ using an oracle terrain classifier (Fig~\ref{fig:fig2}a). From a \DIFdelbegin \DIFdel{default }\DIFdelend walking policy, we utilise a \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend that prepares the robot for the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend (Fig~\ref{fig:fig2}b)). When to switch from the \DIFdelbegin \DIFdel{Setup Policy to the Target Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy to the target policy }\DIFaddend is also a learned output of the \DIFdelbegin \DIFdel{Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policy}\DIFaddend . We first study the traversal of a single difficult terrain artifact that requires walking on a flat surface and performing a jump. We then consider several diverse terrain types (gaps, hurdles, stairs, and \DIFdelbegin \DIFdel{steps}\DIFdelend \DIFaddbegin \DIFadd{stepping stones}\DIFaddend ). The state provided to each policy is $s_t=[rs_t, I_t]$, where $rs_{t}$ is the robot state and $I_t$ is the perception input at time $t$. 

\noindent\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}, s_{right}, s_{left} ]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot \DIFdelbegin \DIFdel{, respectively }\DIFdelend (four Boolean contact points per foot), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the \DIFdelbegin \DIFdel{body Centre of Mass (CoM)}\DIFdelend \DIFaddbegin \DIFadd{robot body}\DIFaddend , $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the \DIFdelbegin \DIFdel{CoM }\DIFdelend \DIFaddbegin \DIFadd{robot body }\DIFaddend and $h_{CoM,t}$ is the height of the robot from the walking surface. $s_{right}$ and $s_{left}$ are Boolean indicators of which foot is in the swing phase, and is updated when the current swing foot makes contact with the ground. \DIFdelbegin \DIFdel{All angles except joint angles are represented in the world coordinate frame}\DIFdelend \DIFaddbegin \DIFadd{Robot body rotations are provided as Euler angles}\DIFaddend . In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\noindent\textbf{Perception}: Perception is a depth sensor mounted to the robot base, with a resolution of $[48,48,1]$\DIFaddbegin \DIFadd{, and field of view of 60 degrees}\DIFaddend . Each pixel is a continuous value scaled between $0-1$, measuring a distance between 0.25 and $\SI{2}{\metre}$ from the robot base. The sensor moves with the body in translation and yaw, we provide an artificial gimbal to keep the sensor fixed in roll and pitch. The sensor is pointed at the robot's feet (\DIFaddbegin \DIFadd{downwards 60 degrees so }\DIFaddend the feet are visible) and covers at least two steps in front of the robot~\cite{zaytsev_two_2015}. We reduce the sampling rate of the perception to $\SI{20}{\hertz}$ (reducing computational complexity), where the simulator operates at $\SI{120}{\hertz}$.

\subsection{Deep Reinforcement Learning for Continuous Control}
\label{sec:ppo}

We consider our task to be a Markov Decision Process $\text{MDP}$, defined by tuple \DIFdelbegin \DIFdel{$\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ }\DIFdelend \DIFaddbegin \DIFadd{$\{\mathcal{S},\mathcal{A}, \mathcal{R}, \mathcal{P}, \gamma\}$ }\DIFaddend where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, \DIFdelbegin \DIFdel{$r_t \in R$ }\DIFdelend \DIFaddbegin \DIFadd{$r_t \in \mathcal{R}$ }\DIFaddend are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. 

The goal of reinforcement learning is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. Actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is \DIFdelbegin \DIFdel{a torque applied to each joint }\DIFdelend \DIFaddbegin \DIFadd{the joint commands}\DIFaddend . Each policy is trained with Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. We use the implementation of PPO from OpenAI Baselines~\cite{dhariwal_openai_2017}.

% We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

% We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[-\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse reduce its probability.

% In practice this loss can be noisy, and result in large updates to the policy. Insteasd we use Proximal Policy Optimisation~\cite{schulman_proximal_2017}, which uses a surrogate loss that is clipped, preventing policy updates that are too large. We also use Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}. 


\subsection{Training Setup Policies}
\label{sec:setup}

For each target terrain type we train a \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend with the purpose of bridging the trajectories of a default walking policy and the \DIFdelbegin \DIFdel{policy for }\DIFdelend \DIFaddbegin \DIFadd{behaviour for traversing }\DIFaddend the upcoming terrain\DIFdelbegin \DIFdel{condition}\DIFdelend . The algorithm for training each \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend is shown in Algorithm~\ref{alg:setup}. 

\textbf{Default Policy}: 
The \DIFdelbegin \DIFdel{Default Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy }\DIFaddend is a pre-trained policy designed to walk on a flat surface. When training a \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend we always begin with the \DIFdelbegin \DIFdel{Default Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy }\DIFaddend until the terrain artifact is detected by an oracle. Once the terrain has been traversed, we switch back to the \DIFdelbegin \DIFdel{Default Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy }\DIFaddend when a termination criteria is reached ($\tau_\theta$, defined below). We initialise the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend from the default walking policy such that the robot continues to walk towards the obstacle while learning how to prepare for the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend .

\textbf{Setup Policy}: 
When terrain type $i$ is detected, we switch immediately from the \DIFdelbegin \DIFdel{Default Policy to the Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy to the setup policy }\DIFaddend for terrain type $i$, denoted as $\pi_\phi^i$. While training we are given access to an oracle terrain detector that indicates when the robot is a fixed distance from the terrain artifact. The \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend outputs joint torques $a_i$, and switch condition $\tau_\phi$. If the switch condition is met, we immediately switch to the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend .

\textbf{Target Policy}: 
The \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend for terrain type $i$, denoted as $\pi_\theta^i$, is trained with curriculum learning following the method outlined in \DIFdelbegin \DIFdel{our previous }\DIFdelend \DIFaddbegin \DIFadd{prior }\DIFaddend work~\cite{tidd_guided_2020}. We also define a termination condition $\tau_\theta$ that denotes switching from the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend back to the \DIFdelbegin \DIFdel{Default Policy}\DIFdelend \DIFaddbegin \DIFadd{default policy}\DIFaddend . For the the termination condition to be reached\DIFaddbegin \DIFadd{, }\DIFaddend the robot must \DIFdelbegin \DIFdel{be have successfully traversed the terrain artifact, }\DIFdelend \DIFaddbegin \DIFadd{successfully traverse the terrain obstacle and }\DIFaddend have both feet in contact with the ground\DIFdelbegin \DIFdel{plane, and a positive forward velocity $vx$}\DIFdelend . This condition is the same for all artifact types.
%DIF >  , and a positive forward velocity $vx$.

\textbf{Setup Policy Reward}: 
We design a reward function to motivate the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend to transition the robot from states visited by the \DIFdelbegin \DIFdel{Default Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy }\DIFaddend to states required by the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend . We note the value function of the \DIFdelbegin \DIFdel{Target Policy, $\hat{V}(s_t) = \sum_{t=0}^{T}\gamma^tr_t$}\DIFdelend \DIFaddbegin \DIFadd{target policy, $V^{\pi_\theta^i}(s_t) = \sum_{t=0}^{T}\gamma^tr_t$}\DIFaddend , (where $r_t$ is the original reward afforded by the environment for the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend ), provides an estimate of what return we can expect if we run the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend from $s_t$. However, value functions are notoriously \DIFdelbegin \DIFdel{over optimistic }\DIFdelend \DIFaddbegin \DIFadd{over-optimistic }\DIFaddend for states that have not been visited~\cite{haarnoja_soft_2018} (such as those we might experience by running the \DIFdelbegin \DIFdel{Default Policy}\DIFdelend \DIFaddbegin \DIFadd{default policy}\DIFaddend ).

The advantage is a zero centered \DIFdelbegin \DIFdel{estimate of the effect of running action $a_t\sim\pi_\theta^i (s_t)$, given by the advantage for the Target Policy}\DIFdelend \DIFaddbegin \DIFadd{calculation of how much better or worse policy $\pi$ performs compared to the value function prediction ${V}^\pi(s_t)$:
}

\begin{equation}
    \DIFadd{A^\pi(s_t, a_t) = R_t - V^\pi(s_t)
}\end{equation}

\DIFadd{where $R_t$ is sum of future rewards from time $t$ running policy $\pi$.
}

\DIFadd{We estimate the advantage using the temporal difference (TD) error with the value function of the target policy $\pi_\theta^i$}\DIFaddend :

\begin{equation}
    \hat{A}\DIFaddbegin \DIFadd{^{\pi_\theta^i}}\DIFaddend (s_t, a_t) = r_t + \gamma \DIFdelbegin %DIFDELCMD < \hat{V}%%%
\DIFdelend \DIFaddbegin \DIFadd{V^{\pi_\theta^i}}\DIFaddend (s\DIFdelbegin \DIFdel{_{t+1)} }\DIFdelend \DIFaddbegin \DIFadd{_{t+1}) }\DIFaddend - \DIFdelbegin %DIFDELCMD < \hat{V}%%%
\DIFdelend \DIFaddbegin \DIFadd{V^{\pi_\theta^i}}\DIFaddend (s_t)
\end{equation}

where $r_t$ is the \DIFdelbegin \DIFdel{Target Policy reward.
(details can be found in our previous work~\mbox{%DIFAUXCMD
\cite{tidd_guided_2020}}\hspace{0pt}%DIFAUXCMD
).
    }\DIFdelend \DIFaddbegin \DIFadd{target policy reward.
}\DIFaddend 

Using advantage \DIFdelbegin \DIFdel{$\hat{A}(s_t, a_t)$ as a confidence for }\DIFdelend \DIFaddbegin \DIFadd{$\hat{A}^{\pi_\theta^i}(s_t, a_t)$ as an indication of }\DIFaddend the accuracy of \DIFdelbegin \DIFdel{$\hat{V}(s_t)$}\DIFdelend \DIFaddbegin \DIFadd{$V^{\pi_\theta^i}(s_t)$}\DIFaddend , we define the reward \DIFdelbegin \DIFdel{from the }\DIFdelend \textbf{Advantage Weighted Target Value}:
\begin{equation}
    \hat{r}_t = ( 1 - \text{min}(\alpha\hat{A}\DIFaddbegin \DIFadd{^{\pi_\theta^i}}\DIFaddend (s_t, a_t)^2,1) ) \cdot \beta\hat{V}\DIFaddbegin \DIFadd{^{\pi_\theta^i}}\DIFaddend (s_t)
    \DIFaddbegin \label{eq:eq1}
\DIFaddend \end{equation}

\DIFdelbegin \DIFdel{Where }\DIFdelend \DIFaddbegin \DIFadd{where }\DIFaddend $\alpha$ and $\beta$ are scaling factors \DIFdelbegin \DIFdel{are }\DIFdelend tuned empirically (set to 0.15 and 0.01 respectively). 

The \DIFdelbegin \DIFdel{Target Policy value function $\hat{V}(s_t)$ }\DIFdelend \DIFaddbegin \DIFadd{target policy value function $V^{\pi_\theta^i}(s_t)$ }\DIFaddend has learned the value for states where the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend has collected experience. Outside of these states, for example when the robot is activating a different policy, we expect the reward provided by the environment $r_t$, and the next state $s_{t+1}$ will not be consistent with what is expected by the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend value function. Therefore, the advantage \DIFdelbegin \DIFdel{$\hat{A}(s_t, a_t)$ }\DIFdelend \DIFaddbegin \DIFadd{$\hat{A}^{\pi_\theta^i}(s_t, a_t)$ }\DIFaddend will not be close to zero, and $\hat{r}_t$ becomes small. Intuitively, for states where the \DIFdelbegin \DIFdel{Target Policy value function $\hat{V}(s_t)$ }\DIFdelend \DIFaddbegin \DIFadd{target policy value function $V^{\pi_\theta^i}(s_t)$ }\DIFaddend is accurate, the \DIFdelbegin \DIFdel{Target Policy advantage $\hat{A}$ }\DIFdelend \DIFaddbegin \DIFadd{target policy advantage $\hat{A}^{\pi_\theta^i}$ }\DIFaddend will be close to zero, thus the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend will learn to maximise \DIFdelbegin \DIFdel{$\hat{V}$}\DIFdelend \DIFaddbegin \DIFadd{$V^{\pi_\theta^i}$}\DIFaddend . States where \DIFdelbegin \DIFdel{$\hat{A}$ }\DIFdelend \DIFaddbegin \DIFadd{$\hat{A}^{\pi_\theta^i}$ }\DIFaddend is far from zero will reduce the effect of an overconfident \DIFdelbegin \DIFdel{$\hat{V}$}\DIFdelend \DIFaddbegin \DIFadd{$V^{\pi_\theta^i}$}\DIFaddend . 

\textbf{Extended Reward}: 
One issue with training \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend is the delayed effect of actions, where once switched to the \DIFdelbegin \DIFdel{Target }\DIFdelend \DIFaddbegin \DIFadd{target }\DIFaddend policy, the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend is no longer acting on the environment or receiving a reward. Once the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend has transitioned to the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend , we must provide the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend with information regarding the performance of the robot since switching. Our method for solving this problem is to provide the additional reward obtained \textit{after} switching, by including an extended reward in the rollout buffer of the \DIFdelbegin \DIFdel{Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policy}\DIFaddend . We add this extended reward to the last \DIFdelbegin \DIFdel{element of the Setup Policy buffer}\DIFdelend \DIFaddbegin \DIFadd{reward received running the setup policy}\DIFaddend : 
\begin{equation}
    % \text{Buffer}[\hat{r}][-1] \mathrel{+}= \hat{r}_t    
    \hat{r}_{final} = \hat{r}_{final} + \hat{r}_t 
\end{equation}
where $\hat{r}_{final}$ is the final reward entry received by the \DIFdelbegin \DIFdel{Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policy before switching}\DIFaddend , and $\hat{r_t}$ is the reward received at time $t$, after the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend has transitioned to the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend . For algorithmic stability, we clear all but the last entry of the buffer after each training update. The \DIFaddbegin \DIFadd{last reward entry of the buffer becomes $\hat{r}_{final}$ for environment steps that continue after training. The }\DIFaddend procedure for training \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend is provided in Algorithm~\ref{alg:setup}. Note that the termination variable $\tau_t$ (line 7) is either $\tau_\phi$ if the \DIFdelbegin \DIFdel{Current Policy is the Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{current policy is the setup policy}\DIFaddend , or $\tau_\theta$ if the \DIFdelbegin \DIFdel{Current Policy is the Target Policy}\DIFdelend \DIFaddbegin \DIFadd{current policy is the target policy}\DIFaddend .

\begin{algorithm}
	\caption{Setup Before Switching} 
	\begin{algorithmic}[1]
      \State Load Target Policy \DIFaddbegin \DIFadd{$\pi_\theta^i$}\DIFaddend . Load Default Policy \DIFaddbegin \DIFadd{$\pi_\theta^j$
      }\DIFaddend \State Initialise Setup Policy \DIFdelbegin \DIFdel{from }\DIFdelend \DIFaddbegin \DIFadd{$\pi_\phi^i$ from the }\DIFaddend Default Policy
      \State Initialise Buffer
        \State Current Policy $\gets$ Default Policy
		\For {$iteration=1,2,\ldots$}
		    \While {not $done$}
    		    \State $a_t, \tau_t \sim $ Current Policy$(s_t)$ %DIF <   \State ($\tau_t = \tau_\theta || \tau_\phi$)
                    \DIFaddbegin \Comment{$\tau$ is $\tau_\phi$ or $\tau_\theta$}
    		  %DIF >   (\tau is either \tau_\phi or \tau_\theta)
    		  %DIF >   \State ($\tau = \tau_\theta || \tau_\phi$)
    		    \DIFaddend %\Comment{$\tau_\theta$ if Current Policy == }
    		    \State $s_{t+1}, r_t, done = env.step(a_t)$
    		    \If{Terrain detected}
    	            \State \DIFdelbegin \DIFdel{$\hat{A}(s_t, a_t) = r_t + \gamma\hat{V}(s_{t+1}) - \hat{V}(s_t)$
                        }\DIFdelend \DIFaddbegin \DIFadd{$\hat{A}^{\pi_\theta^i}(s_t, a_t) = r_t + \gamma V^{\pi_\theta^i}(s_{t+1}) - V^{\pi_\theta^i}(s_t)$
        		    }\DIFaddend \State \DIFdelbegin \DIFdel{$\hat{r}_t = (1 - \alpha\hat{A}(s_t, a_t)^2)\cdot \beta\hat{V}(s_t)$
                        }\DIFdelend \DIFaddbegin \DIFadd{$\hat{r}_t = (1 - \text{min}(\alpha\hat{A}^{\pi_\theta^i}(s_t, a_t)^2, 1))\cdot \beta V^{\pi_\theta^i}(s_t)$
        		    }\DIFaddend \If{Current Policy == Default Policy}
        		        \State Current Policy $\gets$ Setup Policy \DIFaddbegin \DIFadd{$\pi_\phi^i$
        		        }\State \DIFadd{$\tau_t \gets \tau_\phi$
            		}\DIFaddend \ElsIf{Current Policy == Setup Policy}
        		        \State Store $s_t$, $a_t$, $\hat{r}_t$, $\tau_\phi$ into Buffer
                        \If{Buffer Full}
                            \State PPO Training Update
                            \State Clear buffer (except last entry)
                        \EndIf
            		    \If {$\tau_\phi$}
            		        \State Current Policy $\gets$ Target Policy \DIFaddbegin \DIFadd{$\pi_\theta^i$
            		        }\State \DIFadd{$\tau_t \gets \tau_\theta$
            		    }\DIFaddend \EndIf
        			\ElsIf{$\tau_\theta$}
        			    \State Current Policy $\gets$ Default Policy \DIFaddbegin \DIFadd{$\pi_\theta^j$
        		    }\DIFaddend \EndIf
        		    \If{Current Policy != Setup Policy}
        			 %   \State Buffer$[\hat{r}][-1] \mathrel{+}= \hat{r}_t$
        			    \State $\hat{r}_{final} = \hat{r}_{final} + \hat{r}_t$ 
        			\EndIf
        		\EndIf
        		\State $s_t = s_{t+1}$
        	\EndWhile
		\EndFor
	\end{algorithmic} 
\label{alg:setup}
\end{algorithm}
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD <     %%%
\DIFdelend %DIF >  \vspace{15mm}
% \subsection{Terrain Classification}
% \label{sec:classifier}

% Classifier Network \textbf{TBD}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

We evaluate our method with a biped in simulation. Initial evaluations are performed with a single difficult terrain (Sec~\ref{sec:ablation}, Sec~\ref{sec:reward_choice}, Sec~\ref{sec:comparisons}), before adding more behaviours in Sec~\ref{sec:multi_terrain}. The difficult terrain is a sample of flat terrain with a single block \DIFdelbegin \DIFdel{70cm }\DIFdelend \DIFaddbegin \DIFadd{50 cm }\DIFaddend high, and \DIFdelbegin \DIFdel{30cm }\DIFdelend \DIFaddbegin \DIFadd{30 cm }\DIFaddend in length (in the forward direction of the robot), an example is shown in Fig.~\ref{fig:fig1}. We perform training and evaluation on a single terrain sample, starting the robot from a random $x$ (forward direction) uniformly sampled from \DIFdelbegin \DIFdel{$(0.0, 2.2)\si{\meter}$ }\DIFdelend \DIFaddbegin \DIFadd{(0.0, 2.2) $\si{\meter}$ }\DIFaddend before the terrain artifact, $y$ (strafe) uniformly sampled from \DIFdelbegin \DIFdel{$(-0.6, 0.6)\si{\meter}$, and heading }\DIFdelend \DIFaddbegin \DIFadd{(-0.6, 0.6) $\si{\meter}$, and $heading$ }\DIFaddend (yaw) uniformly sampled from \DIFdelbegin \DIFdel{$(-0.3, 0.3)\si{\radian}$}\DIFdelend \DIFaddbegin \DIFadd{(-0.3, 0.3) $\si{\radian}$}\DIFaddend . All experiments \DIFaddbegin \DIFadd{using a single terrain type }\DIFaddend are evaluated by pausing training and performing 100 evaluation runs, and recording both the Success percentage and Distance percentage. Success \% is defined as the average success rate to reach a goal location several meters past the terrain artifact. Distance \% is the \DIFaddbegin \DIFadd{average }\DIFaddend percentage of total \DIFaddbegin \DIFadd{terrain }\DIFaddend distance the agent successfully \DIFdelbegin \DIFdel{traversed of the terrain}\DIFdelend \DIFaddbegin \DIFadd{covered}\DIFaddend .

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effect of Using Initialisation and Extended Reward}
\label{sec:ablation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We perform an ablation to study the effect of initialising the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend from the walking policy, and the effect of extending the reward after the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend has transitioned to the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend . In all experiments the \DIFdelbegin \DIFdel{Default Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy }\DIFaddend is used until the terrain is detected, then the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend is activated until the termination signal $\tau_\phi$ indicates switching to the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend , and $\tau_\theta$ then results in switching back to the \DIFdelbegin \DIFdel{Default Policy}\DIFdelend \DIFaddbegin \DIFadd{default policy}\DIFaddend .

\begin{itemize}[leftmargin=*]

\item\textbf{Without Initialisation:} We evaluate our method without initialising the \DIFdelbegin \DIFdel{Setup Policy from the Default Walk Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policy from the default walking policy}\DIFaddend , i.e. the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend is randomly initialised.

\item\textbf{Without Extended Reward:} We evaluate our method without including the reward after the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend has switched to the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend . 

\item\textbf{Full Method:} Our method uses a \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend initialised from the \DIFdelbegin \DIFdel{Default Walk Policy}\DIFdelend \DIFaddbegin \DIFadd{default walk policy}\DIFaddend , and receives reward signal after the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend has transitioned to the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend . 

\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Initialisation        & 38.8      & 73.2  \\
        Without Extended Reward       & 12.3      & 58.3  \\
        Full Method                          & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study for \DIFdelbeginFL \DIFdelFL{Initialising }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{initialising setup policies }\DIFaddendFL from \DIFdelbeginFL \DIFdelFL{Walk Policy }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{a default walk policy, }\DIFaddendFL and \DIFdelbeginFL \DIFdelFL{Extended Rewards}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{receiving an extended reward}\DIFaddendFL , \DIFdelbeginFL \DIFdelFL{when }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{for }\DIFaddendFL switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:results}
\end{table}

We can see that initialising the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend with the default walking policy and extending the reward improves learning outcomes as shown in Table~\ref{tab:results}, where our method achieves 82.2\% success compared to 38.8\% \DIFdelbegin \DIFdel{(}\DIFdelend without initialisation from the default walking policy \DIFdelbegin \DIFdel{) }\DIFdelend and 12.3\% \DIFdelbegin \DIFdel{(without extended reward)}\DIFdelend \DIFaddbegin \DIFadd{without receiving the extended reward}\DIFaddend . 
% It is worth noting that training without initialisation from the walking policy required many more training steps to reach an asymptotic result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setup Policy Reward Choice}
\label{sec:reward_choice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For training the setup policy, we investigate several options for the reward provided at each timestep. For each reward type we evaluate with three different random seeds, results are shown in Fig~\ref{fig:results}.

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=\columnwidth]{images/results.png}
\hfill
\caption{We investigate several options for the reward function used \DIFdelbeginFL \DIFdelFL{by the Setup Policy }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{to train a setup policy }\DIFaddendFL on the difficult jump terrain. We show the \DIFdelbeginFL \DIFdelFL{percentage of successful runs }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{success rate }\DIFaddendFL (robot reaches several meters after the jump) \DIFdelbeginFL \DIFdelFL{from }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{during training for }\DIFaddendFL three different random seeds.}
\label{fig:results}
% \vspace{-3mm}
\end{figure}

\begin{itemize}[leftmargin=*]
\item\textbf{Original:} The reward afforded by the environment that is used to train the \DIFdelbegin \DIFdel{Target Policy}\DIFdelend \DIFaddbegin \DIFadd{target policy}\DIFaddend : the reward encourages following an expert motion\DIFdelbegin \DIFdel{(See~\mbox{%DIFAUXCMD
\cite{tidd_guided_2020} }\hspace{0pt}%DIFAUXCMD
for details of the reward function)}\DIFdelend . 

\item\textbf{Constant:} At each timestep a constant reward of 1.5 is given.

\item\textbf{Target Torque:} We \DIFaddbegin \DIFadd{encourage the setup policy to }\DIFaddend match the output of the \DIFdelbegin \DIFdel{Target Policy torque }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend by minimising the error\DIFdelbegin \DIFdel{between the Setup Policy and the Target Policy}\DIFdelend : $\exp[-2.0\cdot (\pi_\phi(s_t) - \pi_\theta(s_t))^2]$. 

\item\textbf{Target Value:} We evaluate the effect of using the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend value function as the reward for the \DIFdelbegin \DIFdel{Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policy}\DIFaddend . This is not the same as the original reward, as it is not provided by the environment, but by \DIFdelbegin \DIFdel{$\beta\hat{V}(s_t)$}\DIFdelend \DIFaddbegin \DIFadd{$\beta V^{\pi_\theta^i}(s_t)$}\DIFaddend , where $\beta$ is scaling factor 0.01.
%DIF <   maximising the Target Policy value function 
    %DIF >   maximising the target policy value function 

\item\textbf{Advantage Weighted Target Value:} We evaluate the reward \DIFdelbegin \DIFdel{based on the Target Policy advantage $\hat{A}$ and value function $\hat{V}$: $( 1 - \text{min}(\alpha\hat{A}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}(s_t)$, where $\alpha$ and $\beta$ are scaling factors 0.15 and 0.01 respectively}\DIFdelend \DIFaddbegin \DIFadd{introduced in Equation \ref{eq:eq1}}\DIFaddend .

\end{itemize}

It can be seen from Fig~\ref{fig:results} that a reward using \textbf{Advantage Weighted Target Value} performs better than other reward choices, achieving the highest average success rate (78.7\%). Using the \DIFdelbegin \DIFdel{Target Value }\DIFdelend \DIFaddbegin \DIFadd{target value }\DIFaddend reaches a success rate of 63.9\%. This disparity, and the large variation in the \DIFdelbegin \DIFdel{Target Value }\DIFdelend \DIFaddbegin \DIFadd{target value }\DIFaddend (green line), shows the effect of over estimation bias often seen with value functions, validating our idea that weighting the value by the advantage reduces the effect of this bias when training \DIFdelbegin \DIFdel{Setup Policies}\DIFdelend \DIFaddbegin \DIFadd{setup policies}\DIFaddend .

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparisons}
\label{sec:comparisons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We compare our method with several others, including end to end methods, without using \DIFdelbegin \DIFdel{Setup Policies}\DIFdelend \DIFaddbegin \DIFadd{setup policies}\DIFaddend , and a method that uses proximity prediction to train a \DIFdelbegin \DIFdel{Transition Policy}\DIFdelend \DIFaddbegin \DIFadd{transition policy}\DIFaddend ~\cite{lee_composing_2019}.

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success\% & Distance\% \\
       \hline
        Single Policy                 & 0.0           & 11.3  \\
        Single Policy With Curriculum & 0.0           &  3.8 \\
        No Setup Policy               & 1.5           & 51.3 \\
        Learn When to Switch          & 0.0           & 44.2  \\
        Proximity Prediction         & 51.3           & 82.4 \\
        Setup Policy (Ours)         & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success and average distance \DIFaddbeginFL \DIFaddFL{of the total length }\DIFaddendFL covered when switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:results_compare}
\end{table}

\begin{itemize}[leftmargin=*]

\begin{figure*}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth]{images/Fig1_2.png}
\includegraphics[width=\textwidth]{images/all.png}
\hfill
\caption{Setup policies \DIFdelbeginFL \DIFdelFL{allow us }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{enable a biped }\DIFaddendFL to transition between \DIFdelbeginFL \DIFdelFL{behaviours to traverse several }\DIFdelendFL complex \DIFaddbeginFL \DIFaddFL{visuo-motor behaviours for traversing a sequence of diverse }\DIFaddendFL terrains.}
\label{fig:multi}
% \vspace{-3mm}
\end{figure*}

\item\textbf{Single Policy:} We train a single end to end policy on the terrain sample.

\item\textbf{Single Policy With Curriculum:} We utilise curriculum learning to train a single end to end policy on the terrain sample (using the method \DIFdelbegin \DIFdel{defined }\DIFdelend \DIFaddbegin \DIFadd{outlined }\DIFaddend in~\cite{tidd_guided_2020}).

\item\textbf{No Setup Policy:} We switch to the \DIFdelbegin \DIFdel{Target Policy from the Default Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy from the default policy }\DIFaddend as soon as the terrain oracle detects the next terrain.

\item\textbf{Learn When to Switch:} We collect data by switching from the \DIFdelbegin \DIFdel{Default Policy to the Target Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy to the target policy }\DIFaddend at random distances from the Jump. We use supervised learning to learn when the robot is in \DIFdelbegin \DIFdel{an }\DIFdelend \DIFaddbegin \DIFadd{a }\DIFaddend suitable state to switch. Details of this method is found in our previous work~\cite{tidd_learning_2021}.

\item\textbf{Proximity Prediction:} We follow the method defined by Lee et al\DIFaddbegin \DIFadd{.}\DIFaddend ~\cite{lee_composing_2019} to train Transition Policies (one for each behaviour) using a proximity predictor function $P(s_t)$. $P(s_t)$ outputs a continuous value that indicates how close the agent is to a configuration that resulted in successful traversal. \DIFdelbegin \DIFdel{$P_(s_t)$ }\DIFdelend \DIFaddbegin \DIFadd{$P(s_t)$ }\DIFaddend is trained using supervised learning from success and failure buffers. The reward used to train the \DIFdelbegin \DIFdel{Transition Policy }\DIFdelend \DIFaddbegin \DIFadd{transition policy }\DIFaddend is the dense reward created by  $P(s_{t+1}) - P(s_{t})$, encouraging the agent to move closer to a \DIFdelbegin \DIFdel{successful switching configuration}\DIFdelend \DIFaddbegin \DIFadd{configuration that results in successful switching}\DIFaddend . For accurate comparison we initialise the transition policy with weights from the walk policy, and utilise the terrain oracle for policy selection (the paper refers to a rule-based meta-policy in place of a terrain oracle~\cite{lee_composing_2019}).

\item\textbf{Setup Policy (Ours):} We follow Algorithm~\ref{alg:setup} to train \DIFdelbegin \DIFdel{Setup Policies}\DIFdelend \DIFaddbegin \DIFadd{setup policies}\DIFaddend . 

\end{itemize}

We can see from Table~\ref{tab:results_compare} that our method for developing \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend performs the best (82.2\% success rate), compared to other methods. A single policy was unable to traverse the difficult jump terrain, even \DIFdelbegin \DIFdel{after }\DIFdelend \DIFaddbegin \DIFadd{with }\DIFaddend an extended learning time and \DIFdelbegin \DIFdel{with }\DIFdelend curriculum learning. \DIFaddbegin \DIFadd{The poor performance of }\textbf{\DIFadd{Single Policy With Curriculum}} \DIFadd{was the result of the robot not progressing through the curriculum, and as a consequence is unable to move without assistive forces. }\DIFaddend We show that \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend are necessary for this problem, with \textbf{No Setup Policy} unable to successfully traverse the terrain (1.5\% success). \textbf{Learning When to Switch} also performed poorly as there are very few states that overlap between the \DIFdelbegin \DIFdel{Default Policy and the Target Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy and the target policy }\DIFaddend for the switch estimator to learn. The \textbf{Proximity Prediction} method was able to successfully traverse the jump 51.3\% of the time. It is worth noting that this method required approximately three times more training episodes than our method to reach the provided results, despite also being initialised from the \DIFdelbegin \DIFdel{Default Policy}\DIFdelend \DIFaddbegin \DIFadd{default policy}\DIFaddend .

These experiments show that for the difficult jump terrain, we require a specialised \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend dedicated to learning the complex jumping behaviour. We show that this specialised policy has a trajectory that does not overlap with the \DIFdelbegin \DIFdel{Default Policy}\DIFdelend \DIFaddbegin \DIFadd{default policy}\DIFaddend , and thus \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend are required. Our method for learning a \DIFdelbegin \DIFdel{Setup Policy method achieves }\DIFdelend \DIFaddbegin \DIFadd{setup policies achieved }\DIFaddend the highest performance on this difficult task.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Multiple Terrain Types}
\label{sec:multi_terrain}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


For our final experiment we train \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend for several additional terrain types. In total we now have modules for jumps, gaps, hurdles, stairs, and \DIFdelbegin \DIFdel{steps}\DIFdelend \DIFaddbegin \DIFadd{stepping stones}\DIFaddend . Fig~\ref{fig:multi} shows a sequence with each terrain type. We follow the pipeline shown in Fig~\ref{fig:fig2}a), where a terrain oracle determines which module should be selected. On selection, the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend is employed until \DIFdelbegin \DIFdel{it determines when to switch to the Target Policy}\DIFdelend \DIFaddbegin \DIFadd{the robot reaches a switch state ($\tau_\phi$), then switching to the target policy}\DIFaddend .
Termination criteria $\tau_\theta$ (introduced in Sec~\ref{sec:method}) determines when to switch back to the \DIFdelbegin \DIFdel{Default Policy for the Jump Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy for the jump obstacle }\DIFaddend only. All other policies resemble the behaviour of the \DIFdelbegin \DIFdel{Default Policy }\DIFdelend \DIFaddbegin \DIFadd{default policy }\DIFaddend on flat terrain, i.e. we continue using the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend after the terrain has been traversed for \DIFdelbegin \DIFdel{Gaps, Hurdles, Stairs, and Steps}\DIFdelend \DIFaddbegin \DIFadd{gaps, hurdles, stairs, and stepping stones}\DIFaddend , until the oracle determines the terrain has changed.

We evaluate with \DIFdelbegin \DIFdel{7 randomly selected terrains types in sequence }\DIFdelend \DIFaddbegin \DIFadd{a sequence of each of the 5 terrain types, randomly shuffled before each run}\DIFaddend . We perform 1000 runs, with a total of \DIFdelbegin \DIFdel{7000 }\DIFdelend \DIFaddbegin \DIFadd{5000 }\DIFaddend various terrain types to be traversed. In Table~\ref{tab:multi_results} we show the \DIFaddbegin \DIFadd{average }\DIFaddend percentage of total distance travelled and success rate with and without using \DIFdelbegin \DIFdel{Setup Policies}\DIFdelend \DIFaddbegin \DIFadd{setup policies}\DIFaddend . A successful run in this scenario is defined as traversing the last terrain in the sequence. Table~\ref{tab:multi_breakdown} shows the failure count for each terrain type.
% Table~\ref{tab:multi_breakdown} shows the individual performance of the agent for each terrain type (number of successful traversals / total traversals).

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \DIFdelbeginFL %DIFDELCMD < \begin{adjustbox}{min width=0.71\columnwidth}
%DIFDELCMD <         %%%
\DIFdelendFL \DIFaddbeginFL \begin{adjustbox}{min width=0.8\columnwidth}
    \DIFaddendFL \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Setup Policies        & \DIFdelbeginFL \DIFdelFL{6.8      }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{1.9      }\DIFaddendFL & \DIFdelbeginFL \DIFdelFL{37.1  }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{36.3  }\DIFaddendFL \\
        %DIF >  With setup policies       & \textbf{26.4}      & \textbf{53.2}  \\
        With Setup Policies       & \textbf{\DIFdelbeginFL \DIFdelFL{26.4}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{71.2}\DIFaddendFL }      & \textbf{\DIFdelbeginFL \DIFdelFL{53.2}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{80.2}\DIFaddendFL }  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success rate and \DIFdelbeginFL \DIFdelFL{percent }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{percentage of the }\DIFaddendFL total \DIFdelbeginFL \DIFdelFL{distance }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{terrain length }\DIFaddendFL travelled \DIFdelbeginFL \DIFdelFL{for }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{from }\DIFaddendFL 1000 episodes of \DIFdelbeginFL \DIFdelFL{7 randomly selected }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{all 5 }\DIFaddendFL terrain types\DIFaddbeginFL \DIFaddFL{, randomly shuffled each episode}\DIFaddendFL .}
    \label{tab:multi_results}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \DIFdelbeginFL %DIFDELCMD < \begin{adjustbox}{min width=0.95\columnwidth}
%DIFDELCMD <         %%%
\DIFdelendFL \DIFaddbeginFL \begin{adjustbox}{min width=0.9\columnwidth}
    \DIFaddendFL \begin{tabular}{cccccc}
                                      & Jump & Gap & Hurdle & Stairs & Steps \\
      \hline
        %DIF >  Without setup policies       & 710      & 90  & \textbf{43} &  \textbf{20} & \textbf{90}  \\
        Without Setup Policies       & \DIFdelbeginFL \DIFdelFL{710      }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{782      }\DIFaddendFL & \DIFdelbeginFL \DIFdelFL{90  }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{52  }\DIFaddendFL & \textbf{\DIFdelbeginFL \DIFdelFL{43}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{36}\DIFaddendFL } &  \textbf{\DIFdelbeginFL \DIFdelFL{20}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{31}\DIFaddendFL } & \textbf{\DIFdelbeginFL \DIFdelFL{90}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{86}\DIFaddendFL }  \\
        %DIF >  With setup policies        & \textbf{420}      & \textbf{70}  & 73 & 36 & 144 \\
        With Setup Policies        & \textbf{\DIFdelbeginFL \DIFdelFL{420}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{36}\DIFaddendFL }      & \textbf{\DIFdelbeginFL \DIFdelFL{70}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{48}\DIFaddendFL }  & \DIFdelbeginFL \DIFdelFL{73 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{43 }\DIFaddendFL & \DIFdelbeginFL \DIFdelFL{36 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{65 }\DIFaddendFL & \DIFdelbeginFL \DIFdelFL{144 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{96 }\DIFaddendFL \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Number of failures by terrain type from 1000 episodes of \DIFdelbeginFL \DIFdelFL{7 randomly selected }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{all 5 }\DIFaddendFL terrain types\DIFaddbeginFL \DIFaddFL{, randomly shuffled each episode}\DIFaddendFL .}
    \label{tab:multi_breakdown}
\end{table}

\DIFaddbegin \begin{table}[h!]
    \vspace{-2mm}
    \centering
    %DIF >  \begin{tabular}{c|c|c|c|c|c}
    %DIF >  \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        %DIF >  \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & \DIFaddFL{Success \% }& \DIFaddFL{Distance \% }\\
       \hline
        \DIFaddFL{Without Setup Policies        }& \DIFaddFL{68.2      }& \DIFaddFL{78.1  }\\
        \DIFaddFL{With Setup Policies       }& \textbf{\DIFaddFL{76.7}}      & \textbf{\DIFaddFL{84.6}}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{\DIFaddFL{Success rate and percentage of the total terrain length travelled from 1000 episodes of 4 terrain types }\textbf{\DIFaddFL{(without the jump terrain)}}\DIFaddFL{, randomly shuffled each episode}}
    \label{tab:multi_results_no_jumps}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{min width=0.82\columnwidth}
    \begin{tabular}{ccccc}
                                      & \DIFaddFL{Gap }& \DIFaddFL{Hurdle }& \DIFaddFL{Stairs }& \DIFaddFL{Steps }\\
      \hline
        \DIFaddFL{Without Setup Policies       }& \DIFaddFL{74  }& \textbf{\DIFaddFL{41}} &  \DIFaddFL{64 }& \DIFaddFL{142  }\\
        \DIFaddFL{With Setup Policies        }&  \textbf{\DIFaddFL{44}}  & \DIFaddFL{51 }& \textbf{\DIFaddFL{49}} & \textbf{\DIFaddFL{90}} \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{\DIFaddFL{Number of failures by terrain type from 1000 episodes of 4 terrain types }\textbf{\DIFaddFL{(without the jump terrain)}}\DIFaddFL{, randomly shuffled each episode.}}
    \label{tab:multi_breakdown_no_jumps}
\end{table}
\newpage
\DIFaddend We can see from Table~\ref{tab:multi_results} that \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend improve the success rate compared to switching policies without the intermediate policy (\DIFdelbegin \DIFdel{26.4}\DIFdelend \DIFaddbegin \DIFadd{71.2}\DIFaddend \% success compared to \DIFdelbegin \DIFdel{6.8}\DIFdelend \DIFaddbegin \DIFadd{1.9}\DIFaddend \%). Table~\ref{tab:multi_breakdown} provides a breakdown of the number of times the robot failed on each terrain. From Table~\ref{tab:multi_breakdown} we can see that \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend are most critical for traversing the difficult jump terrain (reducing the failures from \DIFdelbegin \DIFdel{710 to 420}\DIFdelend \DIFaddbegin \DIFadd{782 to 36}\DIFaddend ), though we also see improvements for gap terrain. 
\DIFdelbegin \DIFdel{These results show the highest failure rate on the multi terrain setup is on the jump terrain, and that there is clear room for improvement on this terrain . While the results show that without setup policies the hurdle, stairs, and steps terrain appear to have less failures than running setup policies, we note that these terrains are visited far less times when running without setup policies due to significant failure with the jumps terrain }\DIFdelend \DIFaddbegin 

\DIFadd{To investigate further, we exclude the jump obstacle from the terrain sequence and still observe a significant benefit using setup policies. Table~\ref{tab:multi_results_no_jumps} shows the performance increase from 68.2\% to 76.7\% of successful traversals for 4 terrain types (excluding the jump obstacle). The stepping stone obstacle had the highest failure rate of the remaining terrain types, investigation is required to improve the setup policies for this terrain (Table~\ref{tab:multi_breakdown_no_jumps})}\DIFaddend .

Despite the clear need for \DIFdelbegin \DIFdel{Setup Policies}\DIFdelend \DIFaddbegin \DIFadd{setup policies}\DIFaddend , we attribute \DIFdelbegin \DIFdel{the relatively low success rate (26.4\%) }\DIFdelend \DIFaddbegin \DIFadd{failures }\DIFaddend to out of distribution states, i.e. the robot visits states in the terrain sequence that it does not experience when training the \DIFdelbegin \DIFdel{Setup Policy. For example, if the robot was on a gap, and using the gaps behaviour, then switches to the jumps Setup Policy to prepare for an upcoming jump, it will not necessarily be in a state that has been seen during training. Training Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policy on the individual terrain types. Training setup policies }\DIFaddend for wider range of states will be investigated in future work. \DIFaddbegin \DIFadd{Furthermore, the performance of behaviours on each individual terrain type could be analysed to improve the generalisation of this method to new behaviours.
}


%DIF >  While the results show that without setup policies the hurdle, stairs, and steps terrain appear to have less failures than running setup policies, we note that these terrains are visited far less times when running without setup policies due to significant failure with the jumps terrain.

%DIF >  These results show the highest failure rate on the multi terrain setup is on the jump terrain, and that there is clear room for improvement on this terrain. 


%DIF >   For example, if the robot was on a gap, and using the gaps behaviour, then switches to the jumps setup policy to prepare for an upcoming jump, it will not necessarily be in a state that has been seen during training.
\DIFaddend 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

It is common practice for legged robots to have separate locomotion policies to traverse different terrain conditions. We propose \DIFdelbegin \DIFdel{Setup Policies that allows }\DIFdelend \DIFaddbegin \DIFadd{setup policies that enable }\DIFaddend smooth transition from \DIFaddbegin \DIFadd{the trajectory of }\DIFaddend one locomotion policy to \DIFdelbegin \DIFdel{a Target Policy for }\DIFdelend \DIFaddbegin \DIFadd{the trajectory of a target policy for traversing difficult terrain with }\DIFaddend a dynamic biped. We use deep reinforcement learning to learn the \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend for which we introduce a novel reward based on the Advantage Weighted Target Value, utilising the scaled value prediction of the \DIFdelbegin \DIFdel{Target Policy }\DIFdelend \DIFaddbegin \DIFadd{target policy }\DIFaddend as the reward for the \DIFdelbegin \DIFdel{Setup Policy}\DIFdelend \DIFaddbegin \DIFadd{setup policy}\DIFaddend . 

In simulation experiments for transitioning from a walking policy to a jumping policy, we show using an in-between \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend yields a higher success rate compared to using a single policy (0$\%$ success rate), or the two policies without the \DIFdelbegin \DIFdel{Setup Policy }\DIFdelend \DIFaddbegin \DIFadd{setup policy }\DIFaddend (from 1.5$\%$ success rate without \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend to 82$\%$). We further show that our method is scalable to other terrain types, and demonstrate the effectiveness of the approach on a sequence of difficult terrain conditions, improving the success rate from \DIFdelbegin \DIFdel{6.8}\DIFdelend \DIFaddbegin \DIFadd{1.9}\DIFaddend $\%$ without \DIFdelbegin \DIFdel{Setup Policies to 26.4}\DIFdelend \DIFaddbegin \DIFadd{setup policies to 71.2}\DIFaddend $\%$.

A limitation of our method is that \DIFdelbegin \DIFdel{the Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend are trained from a default walking policy. We would like to improve the scope of the \DIFdelbegin \DIFdel{Setup Policies }\DIFdelend \DIFaddbegin \DIFadd{setup policies }\DIFaddend such that a wider range of states are funnelled \DIFdelbegin \DIFdel{toward the Target Policy}\DIFdelend \DIFaddbegin \DIFadd{towards the target policy}\DIFaddend . If we allowed further training of the \DIFdelbegin \DIFdel{Target Policies}\DIFdelend \DIFaddbegin \DIFadd{target policies}\DIFaddend , our training method could be used to include more states and improve robustness. \DIFdelbegin \DIFdel{This will be considered }\DIFdelend \DIFaddbegin \DIFadd{The idea of utilising the advantage (estimated by the temporal difference (TD) error) as a confidence metric can be applied generally for region of attraction (RoA) expansion, safe reinforcement learning, and also for blending several behaviours for performing complex composite tasks. These ideas will be explored }\DIFaddend in future work. A significant assumption in this work is that we have access to a terrain oracle, removing this dependency will \DIFdelbegin \DIFdel{also be investigated in future work}\DIFdelend \DIFaddbegin \DIFadd{required as we consider experiments in the real world}\DIFaddend .



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

